KOALA: Empirical Lessons Toward Memory-Efficient and Fast Diffusion Models for Text-to-Image Synthesis

As text-to-image (T2I) synthesis models increase in size, they demand higher inference costs due to the need for more expensive GPUs with larger memory, which makes it challenging to reproduce these models in addition to the restricted access to training datasets. Our study aims to reduce these inference costs and explores how far the generative capabilities of T2I models can be extended using only publicly available datasets and open-source models. To this end, by using the de facto standard text-to-image model, Stable Diffusion XL (SDXL), we present three key practices in building an efficient T2I model: (1) Knowledge distillation: we explore how to effectively distill the generation capability of SDXL into an efficient U-Net and find that self-attention is the most crucial part. (2) Data: despite fewer samples, high-resolution images with rich captions are more crucial than a larger number of low-resolution images with short captions. (3) Teacher: Step-distilled Teacher allows T2I models to reduce the noising steps. Based on these findings, we build two types of efficient text-to-image models, called KOALA-Turbo &-Lightning, with two compact U-Nets (1B & 700M), reducing the model size up to 54% and 69% of the SDXL U-Net. In particular, the KOALA-Lightning-700M is 4x faster than SDXL while still maintaining satisfactory generation quality. Moreover, unlike SDXL, our KOALA models can generate 1024px high-resolution images on consumer-grade GPUs with 8GB of VRAMs (3060Ti). We believe that our KOALA models will have a significant practical impact, serving as cost-effective alternatives to SDXL for academic researchers and general users in resource-constrained environments.

==> figures/comparison_others.tex <==
\begin{figure*}[hbt!]
\centering
\scalebox{0.82}{
\includegraphics[width=\textwidth]{figures/fig_comparison_others.pdf}
% \includegraphics[height=\textheight]{figures/comparison_others.pdf}
}
\caption{\textbf{Comparison between SDM-v2.0 vs. SDXL-Base-1.0 vs. KOALA-700M~(ours).} For each prompt, we use 4 random seeds to generate images, while all models are generated with the same seed for each image.
Follow their inference setups in the official \texttt{huggingface} models of SDM-v2.0~\cite{sdm-v2.0_hf} and SDXL-Base-1.0~\cite{sdxl_hf}, SDM-v2.0 is set to generate with DDIM scheduler~\cite{song2020ddim} and SDXL and ours are set to use Euler discrete scheduler~\cite{karras2022elucidating} with 25 steps. Except for DALLE-2, all samples are generated with 25 denoising steps and the cfg-scale~\cite{ho2022cfg} 7.5.
}
\label{fig:comparison_others}
\vspace{-0.3cm}
\end{figure*}


% \begin{multicols}{2}
% % your text
% \begin{figure*}[htb!]
% \centering
%     \includegraphics[width=\textwidth]{figures/teaser.pdf}
%     \caption{Your Caption}
% \end{figure*}
% \label{fig:teaser}
% % more text
% \end{multicols}

==> figures/dreambooth-1page.tex <==
\begin{figure*}
\centering
\includegraphics[width=0.7\textwidth]{figures/fig_dreambooth_1page.pdf}
\caption{\textbf{Image Generations with Dreambooth+KOALA-700M}.}
\label{fig:dreambooth-1page}
\end{figure*}


==> figures/fig_arch_short.tex <==
\begin{figure*}[t!]
\centering
\includegraphics[width=\textwidth]{figures/arch_short.pdf}
% \vspace{-0.4cm}
\caption{\textbf{Overview of \textcolor{red}{K}n\textcolor{red}{O}wledge-Distill\textcolor{red}{A}tion in \textcolor{red}{LA}tent diffusion model based on SDXL and architecture of \textcolor{red}{KOALA}.} We omit skip connections for simplicity.
% We perform feature distillation in transformer blocks using the output of the self-attention layer. 
We perform feature distillation in transformer blocks using self-attention layers. 
% (see ~\cref{subsec:kd} for details)
}
\vspace{-0.3cm}
\label{fig:arch}
\end{figure*}


==> figures/fig_latency_gpu_11g.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.7\linewidth]{figures/latency_gpu_11g.pdf}
\vspace{-0.2cm}
\caption{\textbf{Latency and memory usage comparison on a consumer-grade GPU~(11GB)}. OOM means \textit{Out-of-Memory}.
We measure the inference time of SDM-v2.0 with $768$px and the other models with $1024$px resolution, using 25 denoising steps.
}
\vspace{-0.3cm}
\label{fig:latency_gpu_11g}
\end{figure}


==> figures/fig_rebuttal_failures.tex <==
\begin{figure*}[h!]
\centering
\includegraphics[width=\textwidth]{figures/fig_rebuttal_failures.pdf}
\caption{\textbf{Failure cases of state-of-the-art SDXL models: SDXL-Base-1.0~\cite{diffusers_sdxl}, SDXL-Lightning~\cite{lin2024lightning}, SDXL-Turbo~\cite{sauer2023sdxl-turbo}, Pixart-$\alpha$~\cite{chen2023pixartalpha}, Pixart-$]\sigma$~\cite{chen2024pixartsigma}, SSD-1B~\cite{gupta2024ssd} with $1024^2$ resolution.} 
}
\label{fig:rebuttal_failures}
    \end{figure*}


==> figures/fig_rebuttal_failures_2_.tex <==
\begin{figure*}[h!]
\centering
\includegraphics[width=\textwidth]{figures/fig_rebuttal_failures(2).pdf}
\caption{
\textbf{Failure cases of state-of-the-art SDXL models: SDXL-Base-1.0, SDXL-Lightning, SDXL-Turbo, Pixart-$\alpha$, Pixart-$\sigma$, SSD-1B.} 
% \textbf{Failure cases of state-of-the-art SDXL models: SDXL-Base-1.0~\cite{diffusers_sdxl}, SDXL-Lightning~\cite{lin2024lightning}, SDXL-Turbo~\cite{sauer2023sdxl-turbo}, Pixart-$\alpha$~\cite{chen2023pixartalpha}, Pixart-$]\sigma$~\cite{chen2024pixartsigma}, SSD-1B~\cite{gupta2024ssd} with $1024^2$ resolution.} 
}
\label{fig:rebuttal_failures(2)}
    \end{figure*}


==> figures/latency_gpu.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.99\textwidth]{figures/fig_latency_gpu.pdf}
\vspace{-0.2cm}
\caption{\textbf{Latency and memory usage comparison on various consumer-grade GPUs}. OOM means \textit{Out-of-Memory}.
We measure the inference time of SDM-v2.0 with $768\times 768$ resolution and the other models with $1024\times1024$.
We use 25 denoising steps and FP16/FP32 precisions.
Note that SDXL-Base cannot operate in the 8GB-GPU.
}
\vspace{-0.3cm}
\label{fig:latency_gpu}
\end{figure*}


==> figures/limitation.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.8\linewidth]{figures/fig_limitation.pdf}
% \vspace{-0.7cm}
\caption{\textbf{Failure cases of KOALA-700M}}
% \vspace{-0.5cm}
\label{fig:limitation}
\end{figure}


% \begin{figure*}[h!]
% \centering
% \includegraphics[width=\textwidth]{figures/limitation.pdf}
% \caption{\textbf{Failure cases of KOALA-700M}}
% \label{fig:limitation}
% \end{figure*}


==> figures/model_spec_comp.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/model_spec_comparison_anno.pdf}
% \vspace{-0.8cm}
\caption{\textbf{U-Net budget comparison.} FLOPs are computed with $1024^2$ resolution and 1 step.
BK-SDXL means the compressed U-Net using BK-SDM~\cite{kim2023bksdm}'s block-level prunning.}
\vspace{-0.5cm}
\label{fig:model_comp}
\end{figure}


==> figures/sota_3d-art.tex <==
\begin{figure*}[h!]
\centering
\includegraphics[width=\textwidth]{figures/fig_sota_3d-art.pdf}
\caption{\textbf{Qualitative comparison with DALLE-2, SDM-v2.0, and SDXL in terms of 3D art}.
% Follow their inference setups in the official \texttt{huggingface} models of SDM-v2.0~\cite{sdm-v2.0_hf} and SDXL-Base-1.0~\cite{sdxl_hf}, SDM-v2.0 is set to generate with DDIM scheduler~\cite{song2020ddim} and SDXL and ours are set to use Euler discrete scheduler~\cite{karras2022elucidating} with 25 steps. Except for DALLE-2, all samples are generated with 25 denoising steps and the cfg-scale~\cite{ho2022cfg} 7.5.
We follow the official inference setups of each model (SDM-v2.0~\cite{sdm-v2.0_hf} and SDXL-Base-1.0~\cite{sdxl_hf}) using \texttt{huggingface}. 
Specifically, SDM-v2.0 is set to generate with DDIM scheduler~\cite{song2020ddim} with 25 steps and SDXL and ours are set to use Euler discrete scheduler~\cite{karras2022elucidating} with 25 steps. And we set all models to use the classifier-free guidance~\cite{ho2022cfg} with 7.5.
}
\label{fig:sota_3d-art}
\end{figure*}


==> figures/sota_comparison.tex <==
\begin{figure*}[h!]
\centering
\scalebox{0.82}{
\includegraphics[width=0.96\textwidth]{figures/fig_sota_comparison.pdf}
}
\caption{\textbf{Qualitative comparison between SDM-v2.0 vs. SDXL-Base-1.0 vs. KOALA-700M~(ours).} For each prompt, we use 4 random seeds to generate images, while all models are generated with the same seed for each image.
SDM-v2.0~\cite{sdm-v2.0_hf} is set to generate with DDIM scheduler~\cite{song2020ddim} and SDXL and ours are set to use Euler discrete scheduler~\cite{karras2022elucidating}. All samples are generated with 25 denoising steps and the cfg-scale~\cite{ho2022cfg} 7.5.
}
\label{fig:sota_comparison}
    \end{figure*}


==> figures/sota_human.tex <==
\begin{figure*}
\centering
\includegraphics[width=\textwidth]{figures/fig_sota_human.pdf}
\caption{\textbf{Qualitative comparison with DALLE-2, SDM-v2.0, and SDXL in terms of portrait photo}.
% Follow their inference setups in the official \texttt{huggingface} models of SDM-v2.0~\cite{sdm-v2.0_hf} and SDXL-Base-1.0~\cite{sdxl_hf}, SDM-v2.0 is set to generate with DDIM scheduler~\cite{song2020ddim} and SDXL and ours are set to use Euler discrete scheduler~\cite{karras2022elucidating} with 25 steps. Except for DALLE-2, all samples are generated with 25 denoising steps and the cfg-scale~\cite{ho2022cfg} 7.5.
We follow the official inference setups of each model (SDM-v2.0~\cite{sdm-v2.0_hf} and SDXL-Base-1.0~\cite{sdxl_hf}) using \texttt{huggingface}. 
Specifically, SDM-v2.0 is set to generate with DDIM scheduler~\cite{song2020ddim} with 25 steps and SDXL and ours are set to use Euler discrete scheduler~\cite{karras2022elucidating} with 25 steps. And we set all models to use the classifier-free guidance~\cite{ho2022cfg} with 7.5.}
\label{fig:sota_human}
\end{figure*}


==> figures/sota_koala-llava-comparison_1_.tex <==
\begin{figure*}
\centering
\includegraphics[width=0.8\textwidth]{figures/sota_koala-llava-comparison(1).pdf}
\caption{\textbf{generated samples with $1024\times1024$ resolution }.
These samples are generated with the prompts in~\cref{sec:app_prompts}.
% We follow the official inference setups of each model (SDM-v2.0~\cite{sdm-v2.0_hf} and SDXL-Base-1.0~\cite{sdxl_hf}) using \texttt{huggingface}. 
% Specifically, SDM-v2.0 is set to generate with DDIM scheduler~\cite{song2020ddim} with 25 steps and SDXL and ours are set to use Euler discrete scheduler~\cite{karras2022elucidating} with 25 steps. And we set all models to use the classifier-free guidance~\cite{ho2022cfg} with 7.5.}
}
\label{fig:sota_koala_llava}
\end{figure*}


==> figures/sota_koala-llava-comparison_2_.tex <==
\begin{figure*}
\centering
\includegraphics[width=0.8\textwidth]{figures/sota_koala-llava-comparison(2).pdf}
\caption{\textbf{generated samples with $1024\times1024$ resolution }.
% These samples are generated with the same prompts in~\cref{fig:teaser} and~\cref{sec:app_prompts}.
These samples are generated with the prompts in~\cref{sec:app_prompts}.
}
\label{fig:sota_koala_llava2}
\end{figure*}


==> figures/sota_painting.tex <==
\begin{figure*}
\centering
\includegraphics[width=\textwidth]{figures/fig_sota_painting.pdf}
\caption{\textbf{Qualitative comparison with DALLE-2, SDM-v2.0, and SDXL in terms of painting}.
% Follow their inference setups in the official \texttt{huggingface} models of SDM-v2.0~\cite{sdm-v2.0_hf} and SDXL-Base-1.0~\cite{sdxl_hf}, SDM-v2.0 is set to generate with DDIM scheduler~\cite{song2020ddim} and SDXL and ours are set to use Euler discrete scheduler~\cite{karras2022elucidating} with 25 steps. Except for DALLE-2, all samples are generated with 25 denoising steps and the cfg-scale~\cite{ho2022cfg} 7.5.
We follow the official inference setups of each model (SDM-v2.0~\cite{sdm-v2.0_hf} and SDXL-Base-1.0~\cite{sdxl_hf}) using \texttt{huggingface}. 
Specifically, SDM-v2.0 is set to generate with DDIM scheduler~\cite{song2020ddim} with 25 steps and SDXL and ours are set to use Euler discrete scheduler~\cite{karras2022elucidating} with 25 steps. And we set all models to use the classifier-free guidance~\cite{ho2022cfg} with 7.5.
}
\label{fig:sota_painting}
\end{figure*}


==> figures/sota_visual-characteristic-1b.tex <==
\begin{figure*}
\centering
\includegraphics[width=\textwidth]{figures/fig_sota_visual-characteristic-1b.pdf}
\caption{\textbf{Generated samples of KOALA-1B and KOALA-700M}.}
\label{fig:sota_visual-characteristic-1b}
\end{figure*}


==> figures/sota_visual-characteristic-1b_2.tex <==
\begin{figure*}
\centering
\includegraphics[width=\textwidth]{figures/fig_sota_visual-characteristic-1b_2.pdf}
\caption{\textbf{Generated samples of KOALA-1B and KOALA-700M}.}
\label{fig:sota_visual-characteristic-1b(2)}
\end{figure*}


==> figures/sota_visual-characteristic.tex <==
\begin{figure*}
\centering
\includegraphics[width=\textwidth]{figures/fig_sota_visual-characteristic.pdf}
\caption{\textbf{The Visual Samples of KOALA-700M}.}
\label{fig:sota_visual-characteristic}
\end{figure*}


==> figures/sota_visual-characteristic_2.tex <==
\begin{figure*}
\centering
\includegraphics[width=0.90\textwidth]{figures/fig_sota_visual-characteristic_2.pdf}
\caption{\textbf{Generated samples of KOALA-700M}. 
% 1st row: various painter styles. 
% 2nd row: various color reflections.
% 3rd row: various seasons.
% 4th row: various times.
Our KOALA-700M model demonstrates faithful visual quality and remarkable controllability across various painter's styles (see the first row), diverse color reflections (see the second row), a range of seasons (see the third row), and different times of day (see the fourth row), in response to the given text prompts.
}
\label{fig:sota_visual-characteristic(2)}
\end{figure*}


==> figures/teaser_short.tex <==
\begin{figure}[t]
\centering
    % \includegraphics[width=0.8\textwidth]{figures/teaser_short2.pdf}
    \includegraphics[width=\linewidth]{figures/teaser_short2.pdf}
\vspace{-0.5cm}
\caption{\textbf{Qualiatative comparison with SDM-v2.0 and SDXL.} 
    With the following settings: FP-16 precision, $\mathbf{1024^2}$ resolution, and 25 denoising steps on NVIDIA 4090 GPU.
    % The prompts and more qualitative comparisons are illustrated in~\cref{sec:app_samples}.
    The prompts are described in~\cref{sec:app_prompts}.
}
\label{fig:teaser}
\vspace{-0.5cm}
\end{figure}



==> sec/2_related_works.tex <==

\section{Related Works}
\label{sec:related_works}

\noindent
% \textbf{Knowledge distillation for efficient T2I diffusion models.}
% Denoising diffusion models~\cite{ho2020ddpm, song2020ddim} dominate the recent state-of-the-art text-to-image (T2I) diffusion models~\cite{rombach2022ldm, ramesh2022dalle2, deepfloyid, saharia2022photorealistic} due to their unprecedented high quality and diversity.
% However, a significant shortcoming of these models is their intensive computational demands during sampling time, which constrains their utility in practical scenarios.

Despite the unprecedented quality of denoising diffusion models~\cite{ho2020ddpm}, their intensive computational demands constrain their utility in practical scenarios.

\textbf{Diffusion step compression}
% To alleviate this problem, many efforts~\cite{salimans2022progressive, meng2023distillation} 
have focused on improving the sampling speed by reducing the number of required sampling steps.
% ~\cite{salimans2022progressive, meng2023distillation}. 
In particular, Salimans et al.~\cite{salimans2022progressive} 
% proposes a concept of \textit{step distillation}, which 
trains a student model with fewer steps, distilled from a pre-trained diffusion model as a teacher model. 
Meng et al.~\cite{meng2023distillation} expand this concept to classifier-free guided diffusion models, facilitating the step distillation for modern text-to-image diffusion models. 
More recently, LCM~\cite{luo2023lcm} shows great generation quality in a few steps by extending the idea of consistency model~\cite{song2023consistency} to latent spaces.
SDXL-Turbo~\cite{sauer2023sdxl-turbo} revisits adversarial learning~\cite{goodfellow2014generative} to improve structural understanding in low-step regimes. 
% Although these methods significantly speed up the inference of models, the hardware prerequisites still pose challenges to practitioners.
However, even with its faster speed, since these methods use SDXL's U-Net as a backbone which requires a large memory size, the hardware prerequisites still pose challenges to practitioners.
% \park{detail.. more paper..}

\textbf{Architectural compression}
% As another line of research, BK-SDM~\cite{kim2023bksdm} 
attempts an architectural compression of diffusion models. 
BK-SDM~\cite{kim2023bksdm} first eliminate redundant network components to construct a shallow model. 
Then, a simple knowledge distillation method~\cite{romero2014featkd1,heo2019featkd2} is used to transfer the knowledge from the original pre-trained diffusion model~(\eg, SDM-v1.4~\cite{sdm-v1.4}). 
Remarkably, this compressed model has achieved substantial reductions in sampling time, GPU memory demands, and storage requirements, with only a modest degradation in performance.
However, their simple block removal method has limitations in compressing more complex and larger U-Net models such as SDXL~\cite{podell2023sdxl}.
Beyond the BK-SDM method, which distills only the last feature at each stage, there is still room for further exploration in distilling knowledge from more complex U-Net in SDXL.
% Also, 
% \park{detail.. more paper..}
% For the first time, our work explores the scalability of architectural compression techniques for recent advances in T2I models (\eg, SDXL~\cite{podell2023sdxl}). 
% We present a comprehensive analysis of critical design elements, such as the architectural framework and supervisory signals. 
% We hope our investigation provides insights to the community. 



==> sec/9_Rebuttal.tex <==
\newpage
\appendix
\onecolumn
\section*{Rebuttal} % 부록 시작을 나타내는 섹션



\input{figures/fig_pcm_comparison}

\input{figures/fig_rebuttal_failures(2)}

==> tables/ab_kd.tex <==
\begin{table*}[t!]
\begin{adjustbox}{width=\textwidth, center}
\begin{subtable}[t]{.1\textwidth}
    \centering
    \begin{tabular}{l c}
    Distill type & HPSv2 \\ \midrule
    SD-loss & 25.53 \\ \hline
    SA	& \textbf{26.74} \\
    CA	& 26.11 \\
    Res	& 26.27 \\
    FFN	& 26.48 \\
    LF	& 26.63 \\
    \end{tabular}
    \caption{\textbf{Distillation type.} }
    \strut
    \strut
    \label{tab:distill_type}
\end{subtable}%
\hspace{0.5em}%
\begin{subtable}[t]{.22\textwidth}
    \centering
    \begin{tabular}{l c}
    Distill loc. & HPSv2 \\ \midrule
    SD-loss & 25.53 \\ \hline
    DW-2	& 25.32 \\
    DW-3	& 25.57 \\
    Mid	& 25.66 \\
    UP-1	& \textbf{26.52} \\
    UP-2	& 26.05 \\
    \end{tabular}
    \caption{\textbf{Distill stage.} }
    \label{tab:distill_loc}
\end{subtable}%
\hspace{0.5em}%
\begin{subtable}[t]{.22\textwidth}
    \centering
    \begin{tabular}{l c}
    SA loc.      & HPSv2 \\ \midrule
    SA-bottom	      & \textbf{26.74} \\
    SA-interleave 	  & 26.58 \\
    SA-up             & 26.48 \\
    \\
    \\
    \\
    \end{tabular}
    \caption{\textbf{SA location.}} 
    \label{tab:sa_loc}
\end{subtable}
\hspace{0.5em}%
\begin{subtable}[t]{.26\textwidth}
    \centering
    \begin{tabular}{l c}
    Combination & HPSv2 \\ \midrule
    Baseline (SA only)	& 26.74 \\ \hline
    SA + LF at DW-1 \& UP-3 	& \textbf{26.98} \\
    SA + Res at DW-1 \& UP-3 	& 26.94 \\
    SA + LF all  & 26.83 \\
    SA + Res all &	26.80 \\
    SA+CA+Res+FFN+LF all & 26.39 \\
    \end{tabular}
    % \caption{\textbf{Combination.} DW-1 \& UP-3 are the highest feature resolution in U-Net. }
    \caption{\textbf{Combination.}}
    \label{tab:combination}
\end{subtable}%
\end{adjustbox}
\vspace{-0.45cm}
\caption{
    \textbf{Analysis of feature level knowledge distillation of U-Net in SDXL~\cite{podell2023sdxl}.} SA, CA, and FFN denote self-attention, cross-attention, and feed-forward net in the transformer block. Res is a convolutional residual block and LF denotes the last feature~(same in BK~\cite{kim2023bksdm}). For the ablation study, we train our KOALA-1B as student U-Net for 30K iterations with a batch size of 32. 
    % We use HPSv2~\cite{wu2023hpsv2} as a visual aesthetics metric, which is more correlated with human preference than FID~\cite{heusel2017fid}.
}
\vspace{-0.4cm}
\label{tab:ablation}
\end{table*}

==> tables/ab_kd2.tex <==
% \begin{table*}[ht]
% \centering


% % Adjust the overall font size of the table if needed to fit the page width
% \footnotesize % You can use \tiny, \small, \footnotesize, \scriptsize etc.

% % Ensure that the set of tables does not exceed the text width
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{cccc}
% % Model depth table
% \begin{minipage}[t]{0.24\textwidth}
% \centering
%     \begin{tabular}{lcc}
%     Distill type & HPSv2v2 & CS \\ \midrule
%     SD-loss & 25.53 \\ 
%     SA	& \textbf{26.74} \\
%     CA	& 26.11 \\
%     Res	& 26.27 \\
%     FFN	& 26.48 \\
%     LF~(BK-SDM)	& 26.63 \\
%     \end{tabular}
%     \caption*{\footnotesize\textbf{Distillation type.} }
%     \label{tab:distill_type}
% \end{minipage}
% &
% % Model width table
% \begin{minipage}[t]{0.24\textwidth}
% \centering
%     \begin{tabular}{lcc}
%     Distill loc. & HPSv2v2 & CS \\ \midrule
%     SD-loss & 25.53 \\
%     DW-2	& 25.32 \\
%     DW-3	& 25.57 \\
%     Mid	& 25.66 \\
%     UP-1	& \textbf{26.52} \\
%     UP-2	& 26.05 \\
%     \end{tabular}
%     \caption*{\footnotesize\textbf{Distill stage.} We distill the SA feature at only each stage. }
%     \label{tab:distill_loc}
% \end{minipage}
% &
% % Training epochs table
% \begin{minipage}[t]{0.24\textwidth}
% \centering
%     \begin{tabular}{lcc}
%     SA loc.      & HPSv2v2 & CS \\ \midrule
%     SA-bottom	      & \textbf{26.74} \\
%     SA-interleave 	  & 26.58 \\
%     SA-up             & 26.48 \\
%       \\
%       \\
%       \\
%     \end{tabular}
%     \caption*{\textbf{SA locations} to distill from a transformer block with a depth of 10 in Teacher U-Net in SDXL.} 
%     \label{tab:sa_loc}
% \end{minipage}
% &
% % Diffusion steps table
% \begin{minipage}[t]{0.24\textwidth}
% \centering
%     \begin{tabular}{lcc}
%     Combination & HPSv2v2 & CS\\ \midrule
%     Baseline (SA only)	& 26.74 \\
%     SA + LF \tiny{at DW-1 \& UP-3} 	& \textbf{26.98} \\
%     SA + Res \tiny{at DW-1 \& UP-3} 	& 26.94 \\
%     SA + LF \tiny{all}  & 26.83 \\
%     SA + Res \tiny{all} &	26.80 \\
%     % SA+CA+Res+FFN+LF all & 26.39 \\
%     ALL feat. & 26.39 \\
%     \end{tabular}
%     \caption*{\footnotesize\textbf{Combination.} DW-1 \& UP-3 are the highest feature resolution in U-Net. }
%     \label{tab:combination}
% \end{minipage}
% \end{tabular}
% }
% \caption{
%     \textbf{Analysis of feature level knowledge distillation of U-Net in SDXL~\cite{podell2023sdxl}.} SA, CA, and FFN denote self-attention, cross-attention, and feed-forward net in the transformer block. Res is a convolutional residual block and LF denotes the last feature~(same in BK~\cite{kim2023bksdm}). For the ablation study, we train our KOALA-1B as student U-Net for 30K iterations with a batch size of 32. 
%     % We use HPSv2v2~\cite{wu2023HPSv2v2} as a visual aesthetics metric, which is more correlated with human preference than FID~\cite{heusel2017fid}.
% }
% \label{tab:ablation}
% \end{table*}








\begin{table*}[t!]
 \centering
\subfloat[\footnotesize Distillation type.]{
     \label{tab:distill_type}
     \resizebox{0.24\textwidth}{!}{
     \setlength{\tabcolsep}{4pt}
     \def\arraystretch{0.7}
        \small
        \begin{tabular}{lcc}
        Distill type & HPSv2 \\ \midrule
        SD-loss & 25.53 \\  
        SA	& \textbf{26.74} \\
        CA	& 26.11  \\  
        Res	& 26.27  \\
        FFN	& 26.48  \\
        LF	& 26.63  \\
        \end{tabular}
         }
}
% \hspace{-1mm}
\subfloat[\footnotesize Distill stage.]{ 
     \label{tab:distill_loc}%\hspace{-3mm}
     \resizebox{0.24\textwidth}{!}{
     \setlength{\tabcolsep}{5pt}
     \def\arraystretch{0.7}
      \begin{tabular}{lcc}
        Distill loc. & HPSv2  \\ \midrule
        SD-loss & 25.53  \\
        DW-2	& 25.32  \\
        DW-3	& 25.57  \\
        Mid	    & 25.66 \\
        UP-1	& \textbf{26.52}  \\
        UP-2	& 26.05  \\
        \end{tabular}
     }
 }
 % \hspace{-1mm}
 \subfloat[\footnotesize SA location.]{
     \label{tab:sa_loc}%\hspace{-3mm}
     \resizebox{0.24\textwidth}{!}{
     \setlength{\tabcolsep}{5pt}
     \def\arraystretch{0.87}
         \begin{tabular}{lcc}
    SA loc.      & HPSv2 \\ \midrule
    SA-bottom	      & \textbf{26.74} \\
    SA-interleave 	  & 26.58  \\
    SA-up             & 26.48  \\
      \\
      \\
      \\
    \end{tabular}
     }
     }
 \subfloat[\footnotesize Combination.]{
     \label{tab:combination}% \hspace{-3mm}
     \resizebox{0.24\textwidth}{!}{
     \setlength{\tabcolsep}{2pt}
     \def\arraystretch{0.92}
        \begin{tabular}{lcc}
        Combination & HPSv2 \\ \midrule
        Baseline (SA only)	& 26.74 \\
        SA + LF \tiny{at DW-1 \& UP-3} 	& \textbf{26.98} \\
        SA + Res \tiny{at DW-1 \& UP-3} 	& 26.94  \\
        SA + LF \tiny{all}  & 26.83  \\
        SA + Res \tiny{all} &	26.80  \\
        % SA+CA+Res+FFN+LF all & 26.39 \\
        ALL feat. & 26.39 \\
        \end{tabular}
     }
     }
     

% \vspace{3mm}
% \captionsetup{font=footnotesize}
\caption{
    \textbf{Analysis of feature level knowledge distillation of U-Net in SDXL~\cite{podell2023sdxl}.}
    We use two metrics: Human Preference Score~(HPSv2)~\cite{wu2023hpsv2} for visual aesthetics and T2I-CompBench~(CB) for image-text alignment.
    SA, CA, and FFN denote self-attention, cross-attention, and feed-forward net in the transformer block. Res is a convolutional residual block and LF denotes the last feature~(same in BK~\cite{kim2023bksdm}). For the ablation study, we train our KOALA-1B as student U-Net for 30K iterations with a batch size of 32. 
    % We use HPSv2v2~\cite{wu2023HPSv2v2} as a visual aesthetics metric, which is more correlated with human preference than FID~\cite{heusel2017fid}.
}
\vspace{-0.2cm}
\label{tab:ablation}
\end{table*}

==> tables/ab_kd_short.tex <==
\begin{table*}[t!]
% \begin{adjustbox}{width=0.75\textwidth, center}
\begin{subtable}[t]{.1\textwidth}
    % \hspace*{-3.3cm} % Move the table to the left
    \centering
    \begin{tabular}{l c}
    Distill type & HPSv2 \\ \midrule
    SD-loss & 25.53 \\ \hline
    SA	& \textbf{26.74} \\
    CA	& 26.11 \\
    Res	& 26.27 \\
    FFN	& 26.48 \\
    LF~(BK-SDM~\cite{kim2023bksdm})	& 26.63 \\
    \end{tabular}
    \caption{\textbf{Distillation type.} }
    \label{tab:distill_type}
\end{subtable}%
% \hspace*{-1.5cm} % Move the table to the left
\hspace{0.9em}%
\begin{subtable}[t]{.1\textwidth}
    \centering
    \begin{tabular}{l c}
    Distill loc. & HPSv2 \\ \midrule
    SD-loss & 25.53 \\ \hline
    DW-2	& 25.32 \\
    DW-3	& 25.57 \\
    Mid	& 25.66 \\
    UP-1	& \textbf{26.52} \\
    UP-2	& 26.05 \\
    \end{tabular}
    % \caption{\textbf{Distill stage.} We distill the SA feature at only each stage. }
    \caption{\textbf{Distill stage.} }
    \label{tab:distill_loc}
\end{subtable}%
\hfill
% \hspace{0.9em}%
\begin{subtable}[t]{.22\textwidth}
    \centering
    \begin{tabular}{l c}
    SA loc.      & HPSv2 \\ \midrule
    SA-bottom	      & \textbf{26.74} \\
    SA-interleave 	  & 26.58 \\
    SA-up             & 26.48 \\
    \\
    \\
    \\
    \end{tabular}
    % \caption{\textbf{SA locations} to distill from a transformer block with a depth of 10 in Teacher U-Net in SDXL.} 
    \caption{\textbf{SA location.}} 
    \label{tab:sa_loc}
\end{subtable}
\hspace{0.9em}%
\begin{subtable}[t]{.26\textwidth}
    \centering
    \begin{tabular}{l c}
    Combination & HPSv2 \\ \midrule
    Baseline (SA only)	& 26.74 \\ \hline
    SA + LF at DW-1 \& UP-3 	& \textbf{26.98} \\
    SA + Res at DW-1 \& UP-3 	& 26.94 \\
    SA + LF all  & 26.83 \\
    SA + Res all &	26.80 \\
    SA+CA+Res+FFN+LF all & 26.39 \\
    \end{tabular}
    % \caption{\textbf{Combination.} DW-1 \& UP-3 are the highest feature resolution in U-Net. }
    \caption{\textbf{Combination.}}
    \label{tab:combination}
\end{subtable}%
% \end{adjustbox}
\caption{
    \textbf{Analysis of feature level knowledge distillation of U-Net in SDXL~\cite{podell2023sdxl}.} SA, CA, and FFN denote self-attention, cross-attention, and feed-forward net in the transformer block. Res is a convolutional residual block and LF denotes the last feature~(same in BK~\cite{kim2023bksdm}). 
    % We use HPSv2~\cite{wu2023hpsv2} as a visual aesthetics metric, which is more correlated with human preference than FID~\cite{heusel2017fid}.
}
\vspace{-0.4cm}
\label{tab:ablation}
\end{table*}

==> tables/ab_kd_w_cb.tex <==
% \begin{table*}[ht]
% \centering


% % Adjust the overall font size of the table if needed to fit the page width
% \footnotesize % You can use \tiny, \small, \footnotesize, \scriptsize etc.

% % Ensure that the set of tables does not exceed the text width
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{cccc}
% % Model depth table
% \begin{minipage}[t]{0.24\textwidth}
% \centering
%     \begin{tabular}{lcc}
%     Distill type & HPSv2v2 & CS \\ \midrule
%     SD-loss & 25.53 \\ 
%     SA	& \textbf{26.74} \\
%     CA	& 26.11 \\
%     Res	& 26.27 \\
%     FFN	& 26.48 \\
%     LF~(BK-SDM)	& 26.63 \\
%     \end{tabular}
%     \caption*{\footnotesize\textbf{Distillation type.} }
%     \label{tab:distill_type}
% \end{minipage}
% &
% % Model width table
% \begin{minipage}[t]{0.24\textwidth}
% \centering
%     \begin{tabular}{lcc}
%     Distill loc. & HPSv2v2 & CS \\ \midrule
%     SD-loss & 25.53 \\
%     DW-2	& 25.32 \\
%     DW-3	& 25.57 \\
%     Mid	& 25.66 \\
%     UP-1	& \textbf{26.52} \\
%     UP-2	& 26.05 \\
%     \end{tabular}
%     \caption*{\footnotesize\textbf{Distill stage.} We distill the SA feature at only each stage. }
%     \label{tab:distill_loc}
% \end{minipage}
% &
% % Training epochs table
% \begin{minipage}[t]{0.24\textwidth}
% \centering
%     \begin{tabular}{lcc}
%     SA loc.      & HPSv2v2 & CS \\ \midrule
%     SA-bottom	      & \textbf{26.74} \\
%     SA-interleave 	  & 26.58 \\
%     SA-up             & 26.48 \\
%       \\
%       \\
%       \\
%     \end{tabular}
%     \caption*{\textbf{SA locations} to distill from a transformer block with a depth of 10 in Teacher U-Net in SDXL.} 
%     \label{tab:sa_loc}
% \end{minipage}
% &
% % Diffusion steps table
% \begin{minipage}[t]{0.24\textwidth}
% \centering
%     \begin{tabular}{lcc}
%     Combination & HPSv2v2 & CS\\ \midrule
%     Baseline (SA only)	& 26.74 \\
%     SA + LF \tiny{at DW-1 \& UP-3} 	& \textbf{26.98} \\
%     SA + Res \tiny{at DW-1 \& UP-3} 	& 26.94 \\
%     SA + LF \tiny{all}  & 26.83 \\
%     SA + Res \tiny{all} &	26.80 \\
%     % SA+CA+Res+FFN+LF all & 26.39 \\
%     ALL feat. & 26.39 \\
%     \end{tabular}
%     \caption*{\footnotesize\textbf{Combination.} DW-1 \& UP-3 are the highest feature resolution in U-Net. }
%     \label{tab:combination}
% \end{minipage}
% \end{tabular}
% }
% \caption{
%     \textbf{Analysis of feature level knowledge distillation of U-Net in SDXL~\cite{podell2023sdxl}.} SA, CA, and FFN denote self-attention, cross-attention, and feed-forward net in the transformer block. Res is a convolutional residual block and LF denotes the last feature~(same in BK~\cite{kim2023bksdm}). For the ablation study, we train our KOALA-1B as student U-Net for 30K iterations with a batch size of 32. 
%     % We use HPSv2v2~\cite{wu2023HPSv2v2} as a visual aesthetics metric, which is more correlated with human preference than FID~\cite{heusel2017fid}.
% }
% \label{tab:ablation}
% \end{table*}








\begin{table*}[t!]
 \centering
\subfloat[\footnotesize Distillation type.]{
     \label{tab:distill_type}
     \resizebox{0.24\textwidth}{!}{
     \setlength{\tabcolsep}{4pt}
     \def\arraystretch{0.7}
        \small
        \begin{tabular}{lcc}
        Distill type & HPSv2 & CB \\ \midrule
        SD-loss & 25.53 & 0.2693 \\  
        SA	& \textbf{26.74} & \textbf{0.3237} \\
        CA	& 26.11 & 0.2659 \\  
        Res	& 26.27 & 0.3069 \\
        FFN	& 26.48 & 0.2379 \\
        LF	& 26.63 & 0.3128 \\
        \end{tabular}
         }
}
% \hspace{-1mm}
\subfloat[\footnotesize Distill stage.]{ 
     \label{tab:distill_loc}%\hspace{-3mm}
     \resizebox{0.24\textwidth}{!}{
     \setlength{\tabcolsep}{5pt}
     \def\arraystretch{0.7}
      \begin{tabular}{lcc}
        Distill loc. & HPSv2 & CB \\ \midrule
        SD-loss & 25.53 & 0.2693 \\
        DW-2	& 25.32 & 0.2309 \\
        DW-3	& 25.57 & 0.2590 \\
        Mid	    & 25.66 & 0.2734\\
\vspace{-0.2cm}
        UP-1	& \textbf{26.52} & 0.2606 \\
        UP-2	& 26.05 & \textbf{0.2791} \\
        \end{tabular}
     }
 }
 % \hspace{-1mm}
 \subfloat[\footnotesize SA location.]{
     \label{tab:sa_loc}%\hspace{-3mm}
     \resizebox{0.24\textwidth}{!}{
     \setlength{\tabcolsep}{5pt}
     \def\arraystretch{0.87}
         \begin{tabular}{lcc}
    SA loc.      & HPSv2 & CB \\ \midrule
    SA-bottom	      & \textbf{26.74} & 0.3237 \\
    SA-interleave 	  & 26.58 & \textbf{0.3271} \\
    SA-up             & 26.48 & 0.2943 \\
      \\
      \\
      \\
    \end{tabular}
     }
     }
 \subfloat[\footnotesize Combination.]{
     \label{tab:combination}% \hspace{-3mm}
     \resizebox{0.24\textwidth}{!}{
     \setlength{\tabcolsep}{2pt}
     \def\arraystretch{0.92}
        \begin{tabular}{lcc}
        Combination & HPSv2 & CB\\ \midrule
        Baseline (SA only)	& 26.74 & 0.3237 \\
        SA + LF \tiny{at DW-1 \& UP-3} 	& \textbf{26.98} & \textbf{0.3431} \\
        SA + Res \tiny{at DW-1 \& UP-3} 	& 26.94  & 0.3429 \\
        SA + LF \tiny{all}  & 26.83 & 0.3366 \\
        SA + Res \tiny{all} &	26.80 & 0.3293 \\
        % SA+CA+Res+FFN+LF all & 26.39 \\
        ALL feat. & 26.39 & 0.3079 \\
        \end{tabular}
     }
     }
     

% \vspace{3mm}
% \captionsetup{font=footnotesize}
\caption{
    \textbf{Analysis of feature level knowledge distillation of U-Net in SDXL~\cite{podell2023sdxl}.}
    We use two metrics: Human Preference Score~(HPSv2)~\cite{wu2023hpsv2} for visual aesthetics and T2I-CompBench~(CB) for image-text alignment.
    SA, CA, and FFN denote self-attention, cross-attention, and feed-forward net in the transformer block. Res is a convolutional residual block and LF denotes the last feature~(same in BK~\cite{kim2023bksdm}). For the ablation study, we train our KOALA-1B as student U-Net for 30K iterations with a batch size of 32. 
    % We use HPSv2v2~\cite{wu2023HPSv2v2} as a visual aesthetics metric, which is more correlated with human preference than FID~\cite{heusel2017fid}.
}
\vspace{-0.2cm}
\label{tab:ablation}
\end{table*}

==> tables/arch.tex <==
\begin{table}[t!]
\centering
% \scalebox{0.7}{
\begin{adjustbox}{width=\columnwidth, center}
\normalsize{
\begin{tabular}{l|ccccc}
\toprule
U-Net & SDM-v2.0       & SDXL-1.0         &BK-SDXL & \textbf{KOALA-1B} & \textbf{KOALA-700M} \\ \midrule
\#Param.     & 865M              & 2,567M      &1,717M    & 1,161M             & 782M                 \\
CKPT size & 3.46GB & 10.3GB & 6.8GB & 4.4GB & 3.0GB \\
Tx blocks & {[}1, 1, 1, 1{]} & {[}0, 2, 10{]} & {[}0, 2, 10{]} & {[}0, 2, 6{]}     & {[}0, 2, 5{]} \\
Mid block & \checkmark & \checkmark & \checkmark & \checkmark & \ding{55} \\ 
% Latency & 2.375s & 5.888s & 3.026s & 2.400s \\
Latency & 1.13s & 3.13s & 2.42s & 1.60s & 1.25s \\
\bottomrule
\end{tabular}
}
\end{adjustbox}
% }
\vspace{-0.1cm}
\caption{\textbf{U-Net Comparison.} Tx means Transformer. 
% While SDM-v2.0 uses 4-stage, SDXL and KOALA~(ours) uses 3-stage removing the lowest level~($\times 8$ downsampling). 
SDM-v2.0~\cite{sdm-v2.0} uses $768^2$ resolution, while SDXL and KOALA models use $1024^2$ resolution.
Latency is measured with FP16, and 25 denoising steps in NVIDIA 4090 GPU.
CKPT means the trained checkpoint file.}
\vspace{-0.6cm}
\label{tab:arch}
\end{table} 


% \begin{table}[t]
% \centering
% \begin{adjustbox}{width=\columnwidth, center}
% % \scalebox{0.65}{
% \begin{tabular}{l|cccc}
% \toprule
% U-Net & SDM-v2.0       & SDXL-Base          & \textbf{KOALA-1B} & \textbf{KOALA-700M} \\ \midrule
% Param.     & 865M              & 2,567M          & 1,161M             & 782M                 \\
% CKPT size & 3.46GB & 10.3GB & 4.4GB & 3.0GB \\
% Tx blocks & {[}1, 1, 1, 1{]} & {[}0, 2, 10{]} & {[}0, 2, 6{]}     & {[}0, 2, 5{]} \\
% Mid block & \checkmark & \checkmark & \checkmark & \ding{55} \\ 
% % Latency & 2.375s & 5.888s & 3.026s & 2.400s \\
% Latency & 1.131s & 3.133s & 1.604s & 1.257s \\
% \bottomrule
% \end{tabular}
% % }
% \end{adjustbox}
% \vspace{-0.1cm}
% \caption{\textbf{U-Net Comparison.} Tx means Transformer. 
% % While SDM-v2.0 uses 4-stage, SDXL and KOALA~(ours) uses 3-stage removing the lowest level~($\times 8$ downsampling). 
% SDM-v2.0~\cite{sdm-v2.0} uses $768\times768$ resolution, while SDXL and KOALA models use $1024\times1024$ resolution.
% Latency is measured with FP16-precision, and 25 denoising steps in NVIDIA 4090 GPU~(24GB).
% CKPT means the trained checkpoint file.  }
% \vspace{-0.1cm}

% \label{tab:arch}
% \end{table} 

==> tables/bk_comparison.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[t]
\centering
\begin{adjustbox}{width=0.9\columnwidth, center}
    \begin{tabular}{@{}llcc@{}}
    KD method & Backbone   & HPSv2  & CompBench \\ \midrule
    BK~\cite{kim2023bksdm}        & BK-Small   & 0.2672 & 0.3237    \\
    \textbf{Ours}      & BK-Small   & \textbf{0.2686} & \textbf{0.3417 }   \\
    BK~\cite{kim2023bksdm}        & Koala-1B   & 0.2701  & 0.3599    \\
    \textbf{Ours}      & Koala-1B   & \textbf{0.2715}  & \textbf{0.3712 }  
    \end{tabular}
\end{adjustbox}
\vspace{-0.3cm}
\caption{\textbf{Comparison to BK~\cite{kim2023bksdm}}. All models are trained for 50K iterations same as BK-SDM. We report the average scores of HPSv2 and CompBench.}
\vspace{-0.4cm}
\label{tab:bk_comp}
\end{table}

==> tables/compbench.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[t]
\centering
\scalebox{0.9}{
\begin{tabular}{@{}lccccccc@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Model}} & \multicolumn{3}{c}{Attribute Binding} & \multicolumn{2}{c}{Object Relationship} & \multirow{2}{*}{Complex} & \multirow{2}{*}{Average} \\ \cmidrule(lr){2-6}
\multicolumn{1}{c}{}                       & Color    & Shape   & Texture  & Spatial          & Non-spatial          &                          &                          \\ \midrule
SDM-v1.4\textsuperscript{\textdagger}~\cite{sdm-v1.4}                                   & 0.3765   & 0.3576  & 0.4156   & 0.1246           & 0.3079               & 0.308                    & 0.3150                   \\
SDM-v2.0\textsuperscript{\textdagger}~\cite{sdm-v2.0}                                   & 0.5065   & 0.4221  & 0.4922   & 0.1342           & 0.3096               & 0.3386                   & 0.3672                   \\
DALLE-2\textsuperscript{\textdagger}~\cite{ramesh2022dalle2}                                    & 0.5750   & 0.5464  & 0.6374   & 0.1283           & 0.3043               & 0.3696                   & 0.4268                   \\
SDXL-Base-1.0\textsuperscript{\textdagger}~\cite{podell2023sdxl}                                       & 0.6369   & 0.5408  & 0.5637   & 0.2032           & 0.3110               & 0.4091                   & 0.4441                   \\
\midrule
BK-SDXL-700M                               & 0.5202   & 0.4506  & 0.4564   & 0.1360           & 0.3008               & 0.3699                   & 0.3723                   \\
\textbf{KOALA-700M}                                 & 0.5068   & 0.4731  & 0.4674   & 0.1535           & 0.3008               & 0.3731                   & \textbf{0.3791}          \\
BK-SDXL-1B                                 & 0.4876   & 0.4498  & 0.4578   & 0.1551           & 0.3035               & 0.3777                   & 0.3719                   \\
\textbf{KOALA-1B  }                                 & 0.5223   & 0.5108  & 0.4864   & 0.1563           & 0.3019               & 0.3697                   & \textbf{0.3912}          \\ \bottomrule
\end{tabular}
}
\caption{\textbf{Image-text alignment evaluation} using T2I-CompBench~\cite{huang2023compbench}.
\textsuperscript{\textdagger} denote that the reported results are from the T2I-CompBench~\cite{huang2023compbench} paper.
}
\label{tab:hps}
\end{table*}


% \begin{table*}[t]
% \centering
% \begin{tabular}{lccccccc}
% \toprule
% Model        & Color & Shape & Texture & Spatial & Non-spatial & Complex & Average \\ \midrule
% SDM-v1.4~\cite{sdm-v1.4}     & 0.3765                    & 0.3576                    & 0.4156                      & 0.1246                      & 0.3079                          & 0.308                       & 0.3150                      \\
% SDM-v2.0~\cite{sdm-v2.0}     & 0.5065                    & 0.4221                    & 0.4922                      & 0.1342                      & 0.3096                          & 0.3386                      & 0.3672                      \\
% DALLE-2~\cite{ramesh2022dalle2}      & 0.5750                    & 0.5464                    & 0.6374                      & 0.1283                      & 0.3043                          & 0.3696                      & 0.4268                      \\
% SDXL-Base-1.0~\cite{podell2023sdxl}        & 0.6369                    & 0.5408                    & 0.5637                      & 0.2032                      & 0.3110                          & 0.4091                      & \textbf{0.4441}                      \\
% \midrule
% BK-SDXL-700M & 0.5202                    & 0.4506                    & 0.4564                      & 0.1360                      & 0.3008                          & 0.3699                      & 0.3723                      \\
% \textbf{KOALA-700M}   & 0.5068                    & 0.4731                    & 0.4674                      & 0.1535                      & 0.3008                          & 0.3731                      & \textbf{0.3791}             \\
% BK-SDXL-1B   & 0.4876                    & 0.4498                    & 0.4578                      & 0.1551                      & 0.3035                          & 0.3777                      & 0.3719                      \\
% \textbf{KOALA-1B}     & 0.5223                    & 0.5108                    & 0.4864                      & 0.1563                      & 0.3019                          & 0.3697                      & \textbf{0.3912}             \\ \bottomrule
% \end{tabular}
% \caption{\textbf{Image-text alignment evaluation} using T2I-CompBench~\cite{huang2023compbench}.}
% \label{tab:hps}
% \end{table*}

==> tables/data.tex <==
\begin{table}[t]
\begin{adjustbox}{width=0.8\textwidth, center}
    \begin{tabular}{lccccc}
    \toprule
    % Data                 & \#Samples & avg. Resolution & avg.Prompt Length & HPSv2 & CompBench \\ \midrule
    Data                 & \#Imgs & AR & APL & HPSv2 & CompBench \\ \midrule
    LAION-A-6+~\cite{laion-aesthetics-6plus}           & 8M                   & $580\times676$                             & 13                                 & 27.43                     & 0.3791                        \\
    LAION-A-6+ w/ \texttt{synCap} & 8M                   & $580\times676$                             & 72                                 & 27.61                     & 0.4168                        \\
    LAION-POP~\cite{LAION_POP}            & 491K                     & $1274\times1457$                           & 81                                 & \textbf{27.76}            & \textbf{0.4290}               \\ \bottomrule
    \end{tabular}
\end{adjustbox}
\caption{\textbf{Training Data comparison}. 
AR and APL mean average resolution and average prompt length, respectively. \texttt{synCap} means synthetic captions generated by LLaVA-v1.5~\cite{liu2023improvedllava}}
\end{table}

==> tables/hps.tex <==
\begin{table*}[t]
\vspace{-0.5cm}
\begin{adjustbox}{width=\textwidth, center}
\begin{tabular}{@{}llccccc|ccccccc@{}}
\toprule
\multirow{2}{*}{Model} & \multicolumn{1}{c}{\#Param.}      & \multicolumn{5}{c|}{HPSv2}                                                                                                                             & \multicolumn{3}{c}{Attribute} & \multicolumn{2}{c}{Object Relationship} & \multirow{2}{*}{Complex} & \multirow{2}{*}{Average} \\ \cmidrule(lr){3-12}
                       & \multicolumn{1}{c}{Whole/U-Net} & \multicolumn{1}{c}{Anime} & \multicolumn{1}{c}{Concept-art} & \multicolumn{1}{c}{Paintings} & \multicolumn{1}{c}{Photo} & \multicolumn{1}{c|}{Average} & Color    & Shape   & Texture  & Spatial          & Non-spatial          &                          &                          \\ \midrule
SDM-v1.4~\cite{sdm-v1.4}               & 1.04B 860M                                    & 27.26                     & 26.61                           & 26.66                         & 27.27                     & 26.95                        & 0.3765   & 0.3576  & 0.4156   & 0.1246           & 0.3079               & 0.308                    & 0.3150                   \\
SDM-v2.0~\cite{sdm-v2.0}               & 1.28B 865M                                    & 27.48                     & 26.89                           & 26.86                         & 27.27                     & 27.13                        & 0.5065   & 0.4221  & 0.4922   & 0.1342           & 0.3096               & 0.3386                   & 0.3672                   \\
DALLE-2~\cite{ramesh2022dalle2}                & 6.5B -                                        & 27.34                     & 26.54                           & 26.68                         & 27.24                     & 26.95                        & 0.5750   & 0.5464  & 0.6374   & 0.1283           & 0.3043               & 0.3696                   & 0.4268                   \\
SDXL-Base-1.0~\cite{podell2023sdxl}          & 3.46B 2.6B                                    & 27.69                     & 27.44                           & 27.50                         & 28.29                     & \textbf{27.73}                        & 0.6369   & 0.5408  & 0.5637   & 0.2032           & 0.3110               & 0.4091                   & \textbf{0.4441}                   \\
\midrule
BK-SDM-S~\cite{kim2023bksdm}               & 655M 483M                                     & 26.64                     & 26.77                           & 26.87                         & 26.61                     & 26.72                        & 0.3984   & 0.3783  & 0.4225   & 0.0731           & 0.3003               & 0.3695                   & 0.3237                   \\
\textbf{Ours}-SDM-S             & 655M 483M                                     & 26.73                     & 26.95                           & 27.00                         & 26.74                     & \textbf{26.86}                        & 0.4386   & 0.3950  & 0.4549   & 0.0832           & 0.3007               & 0.3777                   & \textbf{0.3417}          \\
BK-SDM-B~\cite{kim2023bksdm}               & 752M 580M                                     & 27.01                     & 26.64                           & 27.06                         & 26.63                     & 26.84                        & 0.4192   & 0.4096  & 0.4409   & 0.0979           & 0.3077               & 0.3052                   & 0.3301                   \\
\textbf{Ours}-SDM-B             & 752M 580M                                     & 26.79                     & 27.12                           & 27.11                         & 26.79                     & \textbf{26.95}                        & 0.4436   & 0.4338  & 0.4680   & 0.1077           & 0.3090               & 0.3872                   & \textbf{0.3582}          \\
\midrule
BK-SDXL-1B             & 1.68B 782M                                    & 27.52                     & 26.90                           & 27.17                         & 26.87                     & 27.12                        & 0.5202   & 0.4506  & 0.4564   & 0.1360           & 0.3008               & 0.3699                   & 0.3723                   \\
\textbf{KOALA-1B}           & 1.68B 782M                                    & 27.73                     & 27.26                           & 27.61                         & 27.16                     & \textbf{27.44}                        & 0.5068   & 0.4731  & 0.4674   & 0.1535           & 0.3008               & 0.3731                   & \textbf{0.3791}          \\
BK-SDXL-700M           & 2.06B 1.16B                                   & 27.59                     & 27.13                           & 27.17                         & 27.14                     & 27.26                        & 0.4876   & 0.4498  & 0.4578   & 0.1551           & 0.3035               & 0.3777                   & 0.3719                   \\
\textbf{KOALA-700M}         & 2.06B 1.16B                                   & 27.65                     & 27.28                           & 27.58                         & 27.21                     & \textbf{27.43 }                       & 0.5223   & 0.5108  & 0.4864   & 0.1563           & 0.3019               & 0.3697                   & \textbf{0.3912} \\ \bottomrule         
\end{tabular}
\end{adjustbox}
\vspace{-0.2cm}
\caption{\textbf{Visual aesthetics evaluation} using HPSv2~\cite{wu2023hpsv2}~(Left) and \textbf{Image-text alignment evaluation} using T2I-CompBench~\cite{huang2023compbench}~(Right).
Note that BK-SDXL-1B/700M are implemented by ourselves using our efficient U-Net with the BK-SDM~\cite{kim2023bksdm}'s distillation method.
% \textsuperscript{\textdagger} denote that the reported results are from HPSv2~\cite{wu2023hpsv2}.}
}
\vspace{-0.4cm}
\label{tab:hps}
\end{table*}

% \begin{table*}[t]
% \centering
% \scalebox{0.9}{
% % \begin{adjustbox}{width=\columnwidth, center}
% \begin{tabular}{lcccccc}
% \toprule
% Model                                   & \#Param.~(Whole/U-Net)   & Anime & Concept-art & Paintings & Photo & Average \\ \midrule
% SDM-v1.4\textsuperscript{\textdagger}~\cite{sdm-v1.4}                        & 1.04B/860M & 27.26 & 26.61    & 26.66 & 27.27 & 26.95   \\
% SDM-v2.0\textsuperscript{\textdagger}~\cite{sdm-v2.0}                        & 1.28B/865M & 27.48 & 26.89    & 26.86 & 27.27 & 27.13   \\
% DALLE-2\textsuperscript{\textdagger}~\cite{ramesh2022dalle2}                 & 6.5B/-     & 26.54 & 26.68    & 27.24 & 26.95 & 26.95   \\
% SDXL-Base-1.0~\cite{podell2023sdxl}             & 3.46B/2.6B & 27.44 & 27.50    & 28.29 & 27.73 & 27.73   \\ \midrule
% BK-SDM-Small~\cite{kim2023bksdm}                & 655M/483M  & 26.64 & 26.77    & 26.87 & 26.61 & 26.72 \\
% \textbf{Ours}-SDM-Small                         & 655M/483M  & 26.73 & 26.95    & 27.00 & 26.74 & \textbf{26.86} \\
% BK-SDM-Base~\cite{kim2023bksdm}                 & 752M/580M  & 27.06 & 26.63    & 27.01 & 26.64 & 26.84   \\  
% \textbf{Ours}-SDM-Base                          & 752M/580M  & 26.79 & 27.12    & 27.11 & 26.79 & \textbf{26.95}\\
% \midrule
% BK-SDXL-700M~(our impl.)~\cite{kim2023bksdm}         & 1.68B/782M & 27.59 & 27.14       & 27.13     & 27.17 & 27.26   \\
% \textbf{KOALA-700M}~(ours)                      & 1.68B/782M & 27.65 & 27.65       & 27.28     & 27.58 & \textbf{27.43}   \\
% BK-SDXL-1B~(our impl.)~\cite{kim2023bksdm}           & 2.06B/1.16B & 27.52 & 26.87       & 26.9      & 27.17 & 27.12   \\
% \textbf{KOALA-1B}~(ours)                        & 2.06B/1.16B & 27.73 & 27.16       & 27.26     & 27.61 & \textbf{27.44}   \\
% \bottomrule
% \end{tabular}
% }
% % \end{adjustbox}
% \caption{\textbf{Visual aesthetics evaluation} using HPSv2~\cite{wu2023hpsv2}.\textsuperscript{\textdagger} denote that the reported results are from HPSv2~\cite{wu2023hpsv2}.}
% \label{tab:hps}
% \end{table*}

==> tables/hps_compbench.tex <==
\begin{table*}[h]
\vspace{-0.5cm}
\begin{adjustbox}{width=1.0\textwidth, center}
% \begin{tabular}{@{}llccccc|ccccccc@{}}
\begin{tabular}{llccccc|ccccccc}
\toprule
\multirow{2}{*}{Model} & \multicolumn{1}{c}{\#Param.}      & \multicolumn{5}{c|}{HPSv2}                                                                                                                             & \multicolumn{3}{c}{Attribute} & \multicolumn{2}{c}{Object Relationship} & \multirow{2}{*}{Complex} & \multirow{2}{*}{Average} \\ \cmidrule(lr){3-12}
                       & \multicolumn{1}{c}{Whole/U-Net} & \multicolumn{1}{c}{Anime} & \multicolumn{1}{c}{Concept-art} & \multicolumn{1}{c}{Paintings} & \multicolumn{1}{c}{Photo} & \multicolumn{1}{c|}{Average} & Color    & Shape   & Texture  & Spatial          & Non-spatial          &                          &                          \\ \midrule
SDM-v1.4~\cite{sdm-v1.4}               & 1.04B 860M                                    & 27.26                     & 26.61                           & 26.66                         & 27.27                     & 26.95                        & 0.3765   & 0.3576  & 0.4156   & 0.1246           & 0.3079               & 0.308                    & 0.3150                   \\
SDM-v2.0~\cite{sdm-v2.0}               & 1.28B 865M                                    & 27.48                     & 26.89                           & 26.86                         & 27.27                     & 27.13                        & 0.5065   & 0.4221  & 0.4922   & 0.1342           & 0.3096               & 0.3386                   & 0.3672                   \\
DALLE-2~\cite{ramesh2022dalle2}                & 6.5B -                                        & 27.34                     & 26.54                           & 26.68                         & 27.24                     & 26.95                        & 0.5750   & 0.5464  & 0.6374   & 0.1283           & 0.3043               & 0.3696                   & 0.4268                   \\
SDXL-Base-1.0~\cite{podell2023sdxl}          & 3.46B 2.6B                                    & 27.69                     & 27.44                           & 27.50                         & 28.29                     & \textbf{27.73}                        & 0.6369   & 0.5408  & 0.5637   & 0.2032           & 0.3110               & 0.4091                   & \textbf{0.4441}                   \\
\midrule
BK-SDM-S~\cite{kim2023bksdm}               & 655M 483M                                     & 26.64                     & 26.77                           & 26.87                         & 26.61                     & 26.72                        & 0.3984   & 0.3783  & 0.4225   & 0.0731           & 0.3003               & 0.3695                   & 0.3237                   \\
\rowcolor{teagreen}\textbf{Ours}-SDM-S             & 655M 483M                                     & 26.73                     & 26.95                           & 27.00                         & 26.74                     & \textbf{26.86}                        & 0.4386   & 0.3950  & 0.4549   & 0.0832           & 0.3007               & 0.3777                   & \textbf{0.3417}          \\
BK-SDM-B~\cite{kim2023bksdm}               & 752M 580M                                     & 27.01                     & 26.64                           & 27.06                         & 26.63                     & 26.84                        & 0.4192   & 0.4096  & 0.4409   & 0.0979           & 0.3077               & 0.3052                   & 0.3301                   \\
\rowcolor{teagreen}\textbf{Ours}-SDM-B             & 752M 580M                                     & 26.79                     & 27.12                           & 27.11                         & 26.79                     & \textbf{26.95}                        & 0.4436   & 0.4338  & 0.4680   & 0.1077           & 0.3090               & 0.3872                   & \textbf{0.3582}          \\
\midrule
BK-SDXL-700M             & 1.68B 782M                                    & 27.59  & 27.13  & 27.17  & 27.14  & 27.26   & 0.5202   & 0.4506  & 0.4564   & 0.1360           & 0.3008               & 0.3699                   & 0.3723                   \\
\rowcolor{teagreen}\textbf{KOALA-700M}           & 1.68B 782M  & 27.65    & 27.28   & 27.58  & 27.21  & \textbf{27.43}  & 0.5068   & 0.4731  & 0.4674   & 0.1535           & 0.3008               & 0.3731                   & \textbf{0.3791}          \\
BK-SDXL-1B           & 2.06B 1.16B                                   & 27.52 & 26.90  & 27.17  & 26.87  & 27.12  & 0.4876   & 0.4498  & 0.4578   & 0.1551           & 0.3035               & 0.3777                   & 0.3719                   \\
\rowcolor{teagreen}\textbf{KOALA-1B}         & 2.06B 1.16B   & 27.73  & 27.26   & 27.61   & 27.16                & \textbf{27.44}   & 0.5223   & 0.5108  & 0.4864   & 0.1563           & 0.3019               & 0.3697                   & \textbf{0.3912} \\ \bottomrule         
\end{tabular}
\end{adjustbox}
\vspace{-0.2cm}
\caption{\textbf{Visual aesthetics evaluation} using HPSv2~\cite{wu2023hpsv2}~(Left) and \textbf{Image-text alignment evaluation} using T2I-CompBench~\cite{huang2023compbench}~(Right).
Note that BK-SDXL-1B/700M are implemented by ourselves using our efficient U-Net with the BK-SDM~\cite{kim2023bksdm}'s distillation method.
For fair comparison with other methods, we use 50 denoising steps with Euler discrete scheduler~\cite{karras2022elucidating} same as the huggingface's SDXL-Base-1.0 model~\cite{sdxl_hf}.
% \textsuperscript{\textdagger} denote that the reported results are from HPSv2~\cite{wu2023hpsv2}.}
}
% \vspace{-0.4cm}
\label{tab:hps_compbench}
\end{table*}



==> tables/hps_compbench_backup.tex <==
\begin{table*}[t]
\vspace{-0.5cm}
\begin{adjustbox}{width=\textwidth, center}
% \begin{tabular}{@{}llccccc|ccccccc@{}}
\begin{tabular}{llccccc|ccccccc}
\toprule
\multirow{2}{*}{Model} & \multicolumn{1}{c}{\#Param.}      & \multicolumn{5}{c|}{HPSv2}                                                                                                                             & \multicolumn{3}{c}{Attribute} & \multicolumn{2}{c}{Object Relationship} & \multirow{2}{*}{Complex} & \multirow{2}{*}{Average} \\ \cmidrule(lr){3-12}
                       & \multicolumn{1}{c}{Whole/U-Net} & \multicolumn{1}{c}{Anime} & \multicolumn{1}{c}{Concept-art} & \multicolumn{1}{c}{Paintings} & \multicolumn{1}{c}{Photo} & \multicolumn{1}{c|}{Average} & Color    & Shape   & Texture  & Spatial          & Non-spatial          &                          &                          \\ \midrule
SDM-v1.4~\cite{sdm-v1.4}               & 1.04B 860M                                    & 27.26                     & 26.61                           & 26.66                         & 27.27                     & 26.95                        & 0.3765   & 0.3576  & 0.4156   & 0.1246           & 0.3079               & 0.308                    & 0.3150                   \\
SDM-v2.0~\cite{sdm-v2.0}               & 1.28B 865M                                    & 27.48                     & 26.89                           & 26.86                         & 27.27                     & 27.13                        & 0.5065   & 0.4221  & 0.4922   & 0.1342           & 0.3096               & 0.3386                   & 0.3672                   \\
DALLE-2~\cite{ramesh2022dalle2}                & 6.5B -                                        & 27.34                     & 26.54                           & 26.68                         & 27.24                     & 26.95                        & 0.5750   & 0.5464  & 0.6374   & 0.1283           & 0.3043               & 0.3696                   & 0.4268                   \\
SDXL-Base-1.0~\cite{podell2023sdxl}          & 3.46B 2.6B                                    & 27.69                     & 27.44                           & 27.50                         & 28.29                     & \textbf{27.73}                        & 0.6369   & 0.5408  & 0.5637   & 0.2032           & 0.3110               & 0.4091                   & \textbf{0.4441}                   \\
\midrule
BK-SDM-S~\cite{kim2023bksdm}               & 655M 483M                                     & 26.64                     & 26.77                           & 26.87                         & 26.61                     & 26.72                        & 0.3984   & 0.3783  & 0.4225   & 0.0731           & 0.3003               & 0.3695                   & 0.3237                   \\
\rowcolor{teagreen}\textbf{Ours}-SDM-S             & 655M 483M                                     & 26.73                     & 26.95                           & 27.00                         & 26.74                     & \textbf{26.86}                        & 0.4386   & 0.3950  & 0.4549   & 0.0832           & 0.3007               & 0.3777                   & \textbf{0.3417}          \\
BK-SDM-B~\cite{kim2023bksdm}               & 752M 580M                                     & 27.01                     & 26.64                           & 27.06                         & 26.63                     & 26.84                        & 0.4192   & 0.4096  & 0.4409   & 0.0979           & 0.3077               & 0.3052                   & 0.3301                   \\
\rowcolor{teagreen}\textbf{Ours}-SDM-B             & 752M 580M                                     & 26.79                     & 27.12                           & 27.11                         & 26.79                     & \textbf{26.95}                        & 0.4436   & 0.4338  & 0.4680   & 0.1077           & 0.3090               & 0.3872                   & \textbf{0.3582}          \\
\midrule
BK-SDXL-1B             & 1.68B 782M                                    & 27.52                     & 26.90                           & 27.17                         & 26.87                     & 27.12                        & 0.5202   & 0.4506  & 0.4564   & 0.1360           & 0.3008               & 0.3699                   & 0.3723                   \\
\rowcolor{teagreen}\textbf{KOALA-1B}           & 1.68B 782M                                    & 27.73                     & 27.26                           & 27.61                         & 27.16                     & \textbf{27.44}                        & 0.5068   & 0.4731  & 0.4674   & 0.1535           & 0.3008               & 0.3731                   & \textbf{0.3791}          \\
BK-SDXL-700M           & 2.06B 1.16B                                   & 27.59                     & 27.13                           & 27.17                         & 27.14                     & 27.26                        & 0.4876   & 0.4498  & 0.4578   & 0.1551           & 0.3035               & 0.3777                   & 0.3719                   \\
\rowcolor{teagreen}\textbf{KOALA-700M}         & 2.06B 1.16B                                   & 27.65                     & 27.28                           & 27.58                         & 27.21                     & \textbf{27.43 }                       & 0.5223   & 0.5108  & 0.4864   & 0.1563           & 0.3019               & 0.3697                   & \textbf{0.3912} \\ \bottomrule         
\end{tabular}
\end{adjustbox}
\vspace{-0.2cm}
\caption{\textbf{Visual aesthetics evaluation} using HPSv2~\cite{wu2023hpsv2}~(Left) and \textbf{Image-text alignment evaluation} using T2I-CompBench~\cite{huang2023compbench}~(Right).
Note that BK-SDXL-1B/700M are implemented by ourselves using our efficient U-Net with the BK-SDM~\cite{kim2023bksdm}'s distillation method.
For fair comparison with other methods, we use 50 denoising steps with DDIM~\cite{song2020ddim} sampler the same as SDM-v2.0 and SDXL-Base-1.0.
% \textsuperscript{\textdagger} denote that the reported results are from HPSv2~\cite{wu2023hpsv2}.}
}
\vspace{-0.4cm}
\label{tab:hps_compbench}
\end{table*}

==> tables/hps_compbench_icml.tex <==
\begin{table*}[t]
\begin{adjustbox}{width=\textwidth, center}
% \begin{tabular}{@{}llccccc|ccccccc@{}}
\begin{tabular}{llccccc|ccccccc}
\multirow{2}{*}{Model} & \multicolumn{1}{c}{\#Param.}      & \multicolumn{5}{c|}{HPSv2}                                                                                                                             & \multicolumn{3}{c}{Attribute} & \multicolumn{2}{c}{Object Relationship} & \multirow{2}{*}{Complex} & \multirow{2}{*}{Average} \\ \cmidrule(lr){3-12}
                       & \multicolumn{1}{c}{Whole/U-Net} & \multicolumn{1}{c}{Anime} & \multicolumn{1}{c}{Concept-art} & \multicolumn{1}{c}{Paintings} & \multicolumn{1}{c}{Photo} & \multicolumn{1}{c|}{Average} & Color    & Shape   & Texture  & Spatial          & Non-spatial          &                          &                          \\ \midrule
SDM-v1.4$^\dagger$               & 1.04B 860M                                    & 27.26                     & 26.61                           & 26.66                         & 27.27                     & 26.95                        & 0.3765   & 0.3576  & 0.4156   & 0.1246           & 0.3079               & 0.308                    & 0.3150                   \\
SDM-v2.0$^\dagger$               & 1.28B 865M                                    & 27.48                     & 26.89                           & 26.86                         & 27.27                     & 27.13                        & 0.5065   & 0.4221  & 0.4922   & 0.1342           & 0.3096               & 0.3386                   & 0.3672                   \\
DALLE-2$^\dagger$                & 6.5B -                                        & 27.34                     & 26.54                           & 26.68                         & 27.24                     & 26.95                        & 0.5750   & 0.5464  & 0.6374   & 0.1283           & 0.3043               & 0.3696                   & 0.4268                   \\
SDXL-Base-1.0          & 3.46B 2.6B                                    & 27.69                     & 27.44                           & 27.50                         & 28.29                     & \textbf{27.73}                        & 0.6369   & 0.5408  & 0.5637   & 0.2032           & 0.3110               & 0.4091                   & \textbf{0.4441}                   \\
\midrule
\textbf{KOALA-700M}           & 1.68B 782M  & 27.65    & 27.28   & 27.58  & 27.21  & 27.43  & 0.5068   & 0.4731  & 0.4674   & 0.1535           & 0.3008               & 0.3731                   & 0.3791          \\
+ \texttt{LLaVA-synCap} & & 27.79	& 27.43	& 27.85	& 27.27	& 27.59 & 0.5971	&0.5042	&0.5399	&0.1604	&0.3037	&0.3880	&0.4156 \\
\textbf{KOALA-1B}         & 2.06B 1.16B   & 27.73  & 27.26   & 27.61   & 27.16                & 27.44   & 0.5223   & 0.5108  & 0.4864   & 0.1563           & 0.3019               & 0.3697                   & 0.3912 \\ 
+ \texttt{LLaVA-synCap} & & 28.08	& 27.57	& 28.00	& 27.52	& 27.79 & 0.5915	& 0.5189	& 0.5678	& 0.1725	& 0.3046	& 0.3846	& 0.4233 \\
\end{tabular}
\end{adjustbox}
\vspace{-0.2cm}
\caption{
    \textbf{Quantitative comparison to state-of-the-art models} with HPSv2~\cite{wu2023hpsv2}~(Left) for \textbf{visual aesthetics} and with T2I-CompBench~\cite{huang2023compbench}~(Right) for \textbf{Image-text alignment}.
    \texttt{LLaVA-synCap} denotes using synthesized captions by LLaVA.
    $^\dagger$ means reported results in HPSv2 and T2I-Compbench papers.
    For fair comparison with SDXL, we use 50 denoising steps with the Euler discrete scheduler same as the huggingface's SDXL-Base-1.0 model.
    }
\vspace{-0.4cm}
\label{tab:hps_compbench}
\end{table*}



==> tables/hps_compbench_temp.tex <==
\begin{table*}[t]
\vspace{-0.5cm}
\begin{adjustbox}{width=\textwidth, center}
% \begin{tabular}{@{}llccccc|ccccccc@{}}
\begin{tabular}{llccccc|ccccccc}
\toprule
\multirow{2}{*}{Model} & \multicolumn{1}{c}{\#Param.}      & \multicolumn{5}{c|}{HPSv2}                                                                                                                             & \multicolumn{3}{c}{Attribute} & \multicolumn{2}{c}{Object R\begin{table*}[t]
\vspace{-0.5cm}
\begin{adjustbox}{width=\textwidth, center}
% \begin{tabular}{@{}llccccc|ccccccc@{}}
\begin{tabular}{llccccc|ccccccc}
\toprule
\multirow{2}{*}{Model} & \multicolumn{1}{c}{\#Param.}      & \multicolumn{5}{c|}{HPSv2}                                                                                                                             & \multicolumn{3}{c}{Attribute} & \multicolumn{2}{c}{Object Relationship} & \multirow{2}{*}{Complex} & \multirow{2}{*}{Average} \\ \cmidrule(lr){3-12}
                       & \multicolumn{1}{c}{Whole/U-Net} & \multicolumn{1}{c}{Anime} & \multicolumn{1}{c}{Concept-art} & \multicolumn{1}{c}{Paintings} & \multicolumn{1}{c}{Photo} & \multicolumn{1}{c|}{Average} & Color    & Shape   & Texture  & Spatial          & Non-spatial          &                          &                          \\ \midrule
SDM-v1.4~\cite{sdm-v1.4}               & 1.04B 860M                                    & 27.26                     & 26.61                           & 26.66                         & 27.27                     & 26.95                        & 0.3765   & 0.3576  & 0.4156   & 0.1246           & 0.3079               & 0.308                    & 0.3150                   \\
SDM-v2.0~\cite{sdm-v2.0}               & 1.28B 865M                                    & 27.48                     & 26.89                           & 26.86                         & 27.27                     & 27.13                        & 0.5065   & 0.4221  & 0.4922   & 0.1342           & 0.3096               & 0.3386                   & 0.3672                   \\
DALLE-2~\cite{ramesh2022dalle2}                & 6.5B -                                        & 27.34                     & 26.54                           & 26.68                         & 27.24                     & 26.95                        & 0.5750   & 0.5464  & 0.6374   & 0.1283           & 0.3043               & 0.3696                   & 0.4268                   \\
SDXL-Base-1.0~\cite{podell2023sdxl}          & 3.46B 2.6B                                    & 27.69                     & 27.44                           & 27.50                         & 28.29                     & \textbf{27.73}                        & 0.6369   & 0.5408  & 0.5637   & 0.2032           & 0.3110               & 0.4091                   & \textbf{0.4441}                   \\
\midrule
BK-SDM-S~\cite{kim2023bksdm}               & 655M 483M                                     & 26.64                     & 26.77                           & 26.87                         & 26.61                     & 26.72                        & 0.3984   & 0.3783  & 0.4225   & 0.0731           & 0.3003               & 0.3695                   & 0.3237                   \\
\rowcolor{teagreen}\textbf{Ours}-SDM-S             & 655M 483M                                     & 26.73                     & 26.95                           & 27.00                         & 26.74                     & \textbf{26.86}                        & 0.4386   & 0.3950  & 0.4549   & 0.0832           & 0.3007               & 0.3777                   & \textbf{0.3417}          \\
BK-SDM-B~\cite{kim2023bksdm}               & 752M 580M                                     & 27.01                     & 26.64                           & 27.06                         & 26.63                     & 26.84                        & 0.4192   & 0.4096  & 0.4409   & 0.0979           & 0.3077               & 0.3052                   & 0.3301                   \\
\rowcolor{teagreen}\textbf{Ours}-SDM-B             & 752M 580M                                     & 26.79                     & 27.12                           & 27.11                         & 26.79                     & \textbf{26.95}                        & 0.4436   & 0.4338  & 0.4680   & 0.1077           & 0.3090               & 0.3872                   & \textbf{0.3582}          \\
\midrule
BK-SDXL-700M             & 1.68B 782M                                    & 27.59  & 27.13  & 27.17  & 27.14  & 27.26   & 0.5202   & 0.4506  & 0.4564   & 0.1360           & 0.3008               & 0.3699                   & 0.3723                   \\
\rowcolor{teagreen}\textbf{KOALA-700M}           & 1.68B 782M  & 27.65    & 27.28   & 27.58  & 27.21  & \textbf{27.43}  & 0.5068   & 0.4731  & 0.4674   & 0.1535           & 0.3008               & 0.3731                   & \textbf{0.3791}          \\
BK-SDXL-1B           & 2.06B 1.16B                                   & 27.52 & 26.90  & 27.17  & 26.87  & 27.12  & 0.4876   & 0.4498  & 0.4578   & 0.1551           & 0.3035               & 0.3777                   & 0.3719                   \\
\rowcolor{teagreen}\textbf{KOALA-1B}         & 2.06B 1.16B   & 27.73  & 27.26   & 27.61   & 27.16                & \textbf{27.44}   & 0.5223   & 0.5108  & 0.4864   & 0.1563           & 0.3019               & 0.3697                   & \textbf{0.3912} \\ \bottomrule         
\end{tabular}
\end{adjustbox}
\vspace{-0.2cm}
\caption{\textbf{Visual aesthetics evaluation} using HPSv2~\cite{wu2023hpsv2}~(Left) and \textbf{Image-text alignment evaluation} using T2I-CompBench~\cite{huang2023compbench}~(Right).
Note that BK-SDXL-1B/700M are implemented by ourselves using our efficient U-Net with the BK-SDM~\cite{kim2023bksdm}'s distillation method.
For fair comparison with other methods, we use 50 denoising steps with Euler discrete scheduler~\cite{karras2022elucidating} same as the huggingface's SDXL-Base-1.0 model~\cite{sdxl_hf}.
% \textsuperscript{\textdagger} denote that the reported results are from HPSv2~\cite{wu2023hpsv2}.}
}
% \vspace{-0.4cm}
\label{tab:hps_compbench}
\end{table*}

==> tables/main_table_short.tex <==
\begin{table}[t]
    \begin{adjustbox}{width=\linewidth, center}
    \begin{tabular}{lccc}
    Model                                   & Param.(Whole/U-Net) & HPSv2 & CompBench \\ \midrule
    SDM-v1.4~\cite{sdm-v1.4}                & 1.04B/860M          & 26.95 & 0.3150    \\
    SDM-v2.0~\cite{sdm-v2.0}                & 1.28B/865M          & 27.13 & 0.3672    \\
    DALL.E-2~\cite{ramesh2022dalle2}        & 6.5B                & 26.95 & 0.4268    \\
    SDXL-Base~\cite{podell2023sdxl}         & 3.46B/2.6B          & 27.73 & 0.4441    \\ \midrule
    BK-SDXL-700M~\cite{kim2023bksdm}        & 1.68B/782M          & 27.26 & 0.3723    \\
    \rowcolor{teagreen}\textbf{KOALA-700M}  & 1.68B/782M          & 27.43 & 0.3791    \\
    BK-SDXL-1B~\cite{kim2023bksdm}          & 2.06B/1.16B         & 27.12 & 0.3719    \\
    \rowcolor{teagreen}\textbf{KOALA-1B}    & 2.06B/1.16B         & 27.44 & 0.3912    \\ 
    \end{tabular}
    \end{adjustbox}
    \caption{\textbf{Visual aesthetics evaluation} using HPSv2~\cite{wu2023hpsv2}~(Left) and \textbf{Image-text alignment evaluation} using T2I-CompBench~\cite{huang2023compbench}~(Right). 
    % We report average scores of HPSv2 and Compbench~(full scores are detailed in~\cref{sec:app_main_results}).
    \vspace{-0.3cm}
}\label{tab:main_result_short}
\end{table}


==> tables/model_spec.tex <==
\vspace{-0.1cm}
\begin{table}[t]
\centering
\scalebox{0.9}{
    \begin{tabular}{l|ccc}
    \toprule
    SDXL-Base      & Text Enc. & VAE Dec. & U-Net  \\ \midrule
    \#Parameters  & 817M          & 83M          & 2,567M  \\
    Latency~(s) & 0.008        & 0.002       & 3.133  \\ \bottomrule
    \end{tabular}
}
\vspace{-0.1cm}
\caption{\textbf{SDXL-Base-1.0 model budget.} Latency is measured under the image scale of $1024^2$, FP16-precision, and 25 denoising steps in NVIDIA 4090 GPU~(24GB).}
\vspace{-0.3cm}
\label{tab:model_spec}
\end{table}



% \begin{table}[t]
% \begin{adjustbox}{width=\columnwidth, center}
% \begin{tabular}{l|ccc}
% \toprule
% SDXL-Base      & Text Enc. & VAE Dec. & U-Net  \\ \midrule
% \#Parameters  & 817M          & 83M          & 2,567M  \\
% Latency~(s) & 0.008        & 0.002       & 3.133  \\ \bottomrule
% \end{tabular}
% \end{adjustbox}
% \vspace{-0.1cm}
% \caption{\textbf{SDXL-Base-1.0 model budget.} Latency is measured under the image scale of $1024\times 1024$, FP16-precision, and 25 denoising steps in NVIDIA 4090 GPU~(24GB).}
% \vspace{-0.1cm}
% \label{tab:model_spec}
% \end{table}








% \begin{table}[t]
% \begin{adjustbox}{width=\columnwidth, center}
% \begin{tabular}{l|ccc}
% \toprule
% SDXL-Base      & Text Encoder~\cite{ilharco_openclip,radford2021clip} & VAE Decoder~\cite{vae-fp16-fix} & U-Net  \\ \midrule
% SDXL-Base      & Text Encoder~\cite{ilharco_openclip,radford2021clip} & VAE Decoder~\cite{vae-fp16-fix} & U-Net  \\ \midrule
% \#Parameters  & 817M          & 83M          & 2,567M  \\
% Latency~(s) & 0.008        & 0.002       & 3.133  \\ \bottomrule
% \end{tabular}
% \end{adjustbox}
% \vspace{-0.1cm}
% \caption{\textbf{SDXL-Base-1.0 model budget.} Latency is measured under the image scale of $1024\times 1024$, FP16-precision, and 25 denoising steps in NVIDIA 4090 GPU~(24GB).}
% \vspace{-0.1cm}
% \label{tab:model_spec}
% \end{table}




==> tables/pixart.tex <==
\begin{table}[t]
\caption{\textbf{KD location in Diffusion Transformer~(Pixart-$\Sigma$~\cite{chen2024pixartsigma}}.}\label{tab:pixart}
\centering
\begin{adjustbox}{width=0.3\textwidth, center}
    \begin{tabular}{llc}
    KD loc. & HPSv2 \\
    SA & \textbf{25.16} \\
    CA & 24.94 \\
    FF & 24.80 \\
    LF & 21.62 \\
    \end{tabular}
\end{adjustbox}
\end{table}

==> tables/teacher.tex <==
Teacher	HPSv2	CompBench

\begin{table}
    \centering
    \begin{tabular}{ccc}
    SDXL-Base-1.0	& 27.44	& 0.4406 \\
    SDXL-Turbo	& 27.97	& 0.4612 \\
    SDXL-Lightning	& 30.00	 & 0.4467 \\
    \end{tabular}
    \caption{Teacher model comparison.}
    \label{tab:teacher}
\end{table}

==> tables/wrap_data.tex <==
\begin{wraptable}{r}{0.53\linewidth}
\vspace{-8mm}
\caption{\footnotesize{\textbf{Data comparison.} AR and APL mean average resolution and average prompt length, respectively. \texttt{synCap} means synthetic captions generated by LLaVA-v1.5~\cite{liu2023improvedllava}}} \label{tab:data}
    \scalebox{0.67}{
    \begin{tabular}{lccccc}
    \toprule
    Data                 & \#Imgs & AR & APL & HPSv2 & CompBench \\ \midrule
    LAION-A-6+~\cite{laion-aesthetics-6plus}           & 8M                   & $580\times676$                             & 13                                 & 27.43                     & 0.3791                        \\
    + \texttt{synCap} & 8M                   & $580\times676$                             & 72                                 & 27.61                     & 0.4168                        \\
    LAION-POP~\cite{LAION_POP}            & 491K                     & $1274\times1457$                           & 81                                 & \textbf{27.76}            & \textbf{0.4290}               \\ \bottomrule
    \end{tabular}
}
\end{wraptable}

==> tables/wrap_step.tex <==
\begin{wrapfigure}{r}{0.4\textwidth}
    \centering
    \vspace{-8mm}
    \includegraphics[width=\linewidth]{figures/hpsv2_step.pdf}
    \caption{\footnotesize Performance comparisons across denoising steps.}
    \label{fig:poc-memory}
    \vspace{-3mm}
\end{wrapfigure}

==> template/cvpr23/sec_short/0_abstract.tex <==
\begin{abstract}
 % This work does not propose a novel method; instead, it studies a straightforward, empirical yet must-know strategy for compressing Stable Diffusion XL (SDXL) through a knowledge distillation~(KD) scheme.
 This work explores an empirical yet effective strategy for compressing Stable Diffusion XL (SDXL) through a knowledge distillation~(KD) scheme.
 We first design a more efficient U-Net using layer-level pruning. Secondly, we explore how to effectively distill the generation capability of SDXL into an efficient U-Net and eventually identify four essential factors, the core of which is that self-attention is the most crucial part. With our efficient U-Net and self-attention-based KD strategy, we build our efficient text-to-image models, called KOALA-1B~\&-700M, while reducing the model size up to 54\% and 69\% of the SDXL model. In particular, the KOALA-700M is over twice as fast as the SDXL while still maintaining satisfactory generation quality. Moreover, unlike SDXL, our KOALA models can generate 1024px high-resolution images on consumer-grade GPUs (e.g., 8GB VRAM). 
 We hope that thanks to its balanced speed-performance tradeoff, our KOALA models can serve as a cost-effective alternative to SDXL.
 
 % We hope that thanks to its balanced speed-performance tradeoff, our KOALA models can serve as a cost-effective alternative to SDXL for communities, including researchers and general users (e.g., \footnote{\url{https://civitai.com/}}Civitai) in resource-constrained environments.

% Stable diffusion is the mainstay of the text-to-image~(T2I) synthesis in the community due to its generation performance and open-source nature. Recently, Stable Diffusion XL~(SDXL), the successor of stable diffusion, has received a lot of attention due to its significant performance improvements with a higher resolution of $1024\times1024$ and a larger model. However, its increased computation cost and model size require higher-end hardware~(\eg, bigger VRAM GPU) for end-users, incurring higher costs of operation. To address this problem, in this work, we propose an efficient latent diffusion model for text-to-image synthesis obtained by distilling the knowledge of SDXL. To this end, we first perform an in-depth analysis of the denoising U-Net in SDXL, which is the main bottleneck of the model, and then design a more efficient U-Net based on the analysis. Secondly, we explore how to effectively distill the generation capability of SDXL into an efficient U-Net and eventually identify four essential factors, the core of which is that self-attention is the most important part. With our efficient U-Net and self-attention-based knowledge distillation strategy, we build our efficient T2I models, called KOALA-1B~\&-700M, while reducing the model size up to 54\% and 69\% of the original SDXL model. In particular, the KOALA-700M is more than twice as fast as SDXL while still retaining a decent generation quality. We hope that due to its balanced speed-performance tradeoff, our KOALA models can serve as a cost-effective alternative to SDXL in resource-constrained environments.
\end{abstract}



==> template/cvpr23/sec_short/0_meta_data.tex <==
% \title{\includegraphics[width=0.08\linewidth]{figures/koala.pdf}KOALA: Self-Attention Matters in Knowledge Distillation of Latent Diffusion Models for Memory-Efficient and Fast Image Synthesis}
% \title{KOALA: Self-Attention Matters in Knowledge Distillation of Latent Diffusion Models for Memory-Efficient and Fast Image Synthesis}
\title{KOALA: Fast and Memory-Efficient Latent Diffusion Models via Self-Attention Distillation}
% \title{KOALA: An Empirical Study on Compressing Latent Diffusion Model via Knowledge Distillation for Fast Image Synthesis}


\newcommand*{\affaddr}[1]{#1} % No op here. Customize it for different styles.
\newcommand*{\affmark}[1][*]{\textsuperscript{#1}}
\newcommand*{\email}[1]{\texttt{#1}}

\author{%
Youngwan Lee\affmark[1,2]~~~Kwanyong Park\affmark[1]~~~Yoorhim Cho\affmark[3]~~~Yong-Ju Lee\affmark[1]~~~Sung Ju Hwang\affmark[2,4]\\ 
\vspace{-0.1in}
\\
\affaddr{\affmark[1]Electronics and Telecommunications Research Institute~(ETRI), South Korea}\\
\affaddr{\affmark[2]Korea Advanced Institute of Science and Technology~(KAIST), South Korea}\\
\affaddr{\affmark[3]Sookmyung Women's University, South Korea}\\
\affaddr{\affmark[4]DeepAuto.ai, South Korea}\\
\footnotesize{project page: \url{https://youngwanlee.github.io/KOALA/}}
}



==> template/cvpr23/sec_short/1_intro.tex <==
\vspace{-0.2cm}
\section{Introduction}
\label{sec:intro}

% \input{figures/model_spec_comp}


% Background: SDXL의 등장
% Since the emergence of the Stable diffusion models~(SDMs)~\cite{sdm-v2.0, podell2023sdxl} which are based on the latent diffusion model~\cite{rombach2022ldm}, not only text-to-image synthesis has significantly advanced but also derivative applications have been actively developed, such as image editing~\cite{tumanyan2023plug,choi2023custom} and text-to-video generation~\cite{blattmann2023videoldm}.
The emergence of the Stable diffusion models~(SDMs)~\cite{sdm-v2.0, podell2023sdxl} not only advance text-to-image synthesis but also revolutionize derivative applications such as image editing~\cite{tumanyan2023plug,choi2023custom} and text-to-video generation~\cite{blattmann2023videoldm}.
% Furthermore, a more recent version of the stable diffusion model, SDXL~\cite{podell2023sdxl}, demonstrates significantly improved image generation quality with a \textbf{higher resolution} of $\mathbf{1024^2}$, however, its massive computation costs and large model size require expensive hardware equipment and thus incur huge costs.
Furthermore, a more recent version of the SDMs, SDXL~\cite{podell2023sdxl}, enables to generate \textbf{higher resolution} images of $\mathbf{1024^2}$ with significantly improved quality.
However, its massive computation costs and large model size require expensive hardware equipment and thus incur huge costs.

% Motivation (problems to solve, limitations of related works)
% To alleviate this computation burden, the denoising step reduction~(\ie, step-distillation)~\cite{luo2023lcm,sauer2023sdxl-turbo} and architectural model compression methods~\cite{li2023snapfusion,kim2023bksdm} adopt the knowledge distillation~(KD) scheme~\cite{hinton2015outkd,heo2019featkd2} by allowing the model to mimic the output of the SDMs as a teacher model.

To alleviate this computation burden, prior works attempt to either reduce the required sampling steps~(\ie, step-distillation)~\cite{luo2023lcm,sauer2023sdxl-turbo} or compress the model architecture~\cite{li2023snapfusion,kim2023bksdm} through the knowledge distillation~(KD) scheme~\cite{hinton2015outkd,heo2019featkd2}.
% The step-distillation methods~\cite{salimans2022progressive,meng2023distillation,li2023snapfusion} allow the denoised latent of the diffusion model in the early denoising steps to mimic the output in the later denoising steps of the teacher model.
% As an orthogonal work for the architectural model compression, BK-SDM~\cite{kim2023bksdm} exploits KD when compressing the most heavy-weight part, U-Net, in SDM-v1.4~\cite{sdm-v1.4}. 
For the architectural compression, BK-SDM~\cite{kim2023bksdm} exploits KD to compress computationally heavy U-Net~\cite{ronneberger2015uent} part in SDM-v1.4~\cite{sdm-v1.4}. 
% when compressing the most heavy-weight part, U-Net~\cite{ronneberger2015uent}, in SDM-v1.4~\cite{sdm-v1.4}. 
BK-SDM builds a compressed U-Net by simply removing some blocks and allows the compressed U-Net to mimic the last features at each stage of the original U-Net.
% from the teacher model during the pre-training phase.
However, the compression method proposed by BK-SDM achieves a limited compression rate~(33\% in~\cref{tab:arch}) when applied to the larger SDXL than SDM-v1.4, and the strategy of feature distillation for SDXL has \textit{not yet been fully explored}.

\input{figures/teaser_short}

\input{figures/arch_short}

% Our method
In this work, our goal is to build more efficient U-Nets by distilling the generation capability of significantly larger U-Net in SDXL~\cite{podell2023sdxl}.
To this end, we first design two efficient U-Nets, \textbf{KOALA-1B} and \textbf{KOALA-700M}, using not only block removal but also \textit{layer-wise pruning} to reduce the model size of the SDXL's U-Net by up to 54\% and 69\%~(vs. BK's method: 33\%).
Furthermore, we investigate how to effectively distill SDXL as a teacher model and find \textbf{\textit{four essential factors}} for feature-level knowledge distillation.
The core of these findings is that \textit{self-attention} features are the most crucial for distillation.



% Experiments summary
With the proposed strategies, we train an efficient text-to-image synthesis model on top of SDXL~\cite{podell2023sdxl}, called KOALA, by only replacing SDXL's U-Net with our efficient U-Net.
KOALA is trained with $1024^2$ resolution on a smaller \textit{publicly available} LAION-Aesthestics-V2-6+~\cite{laion-aesthetics-6plus}, which has only 8M text-image pairs.
% Recent studies~\cite{kirstain2023pick,wu2023hps,wu2023hpsv2,betzalel2022fid_not_good} have shown that FID~\cite{heusel2017fid} is not well correlated with the fidelity of the generated image, and thus we use two alternative evaluation metrics: Human Preference Score~(HPSv2)~\cite{wu2023hpsv2} for visual aesthetics and T2I-Compbench~\cite{huang2023compbench} for image-text alignment.
% Our efficient KOALA models consistently outperform BK-SDM~\cite{kim2023bksdm}'s KD method in both metrics.
Our efficient KOALA models consistently outperform BK-SDM~\cite{kim2023bksdm}'s KD methods.
Furthermore, our smaller model, KOALA-700M, shows better performance than widely used SDM-v2.0~\cite{sdm-v2.0}, 
% which is one of the most widely used in the community, 
while having a similar model size and inference speed.
Lastly, to validate its practical impact, we perform inference analysis on a variety size of \textbf{\textit{consumer-grade} GPUs}
% with different memory sizes
~(\eg, memory of 8GB, 11GB, and 24GB), and the results show that SDXL cannot be mounted on an 8GB GPU, whereas our KOALA-700M can run on it while still maintaining satisfactory image quality as shown in~\cref{fig:teaser}.



% Contribution Summary
Our main contributions are as follows:
\begin{enumerate}
    % \item We conduct an in-depth architectural analysis of U-Net in SDXL to figure out the model bottleneck. 
    % \item We design two efficient denoising U-Net architectures with model sizes~(1.13B/782M) that are more than twice as compact and faster than SDXL's U-Net~(2.56B), showing that our models can run on an economical GPU with 8 GB of memory.
    \item We design two efficient denoising U-Net with model sizes~(1.13B/782M) that are more than twice as compact and faster than SDXL's U-Net~(2.56B).

    \item We perform a comprehensive analysis of the knowledge distillation strategies for SDXL, finding four essential factors for feature distillation.

    % \item We perform a systemical analysis of inference on consumer-grade GPUs, showing that our KOALA-700M can operate on an economical GPU with 8 GB of memory.
    
    % \item We empirically verify that synthesized captions by a large multimodal model further boost prompt-following ability.
\end{enumerate}

==> template/cvpr23/sec_short/3_method.tex <==
\section{Approach}


% In this section, we first dissect SDXL~\cite{podell2023sdxl} and benchmark its components in terms of model size and computation cost, and then we design a new compact SDXL model called KOALA in~\cref{subsec:arch}.
In this section, we first propose an efficient U-Net architecture in~\cref{subsec:arch}.
% Second, we perform a comprehensive analysis with the proposed efficient U-Net to explore knowledge-distillation strategies in~\cref{subsec:kd}.
Then, we explore how to effectively distill the knowledge from U-Net in SDXL~\cite{podell2023sdxl} into the proposed efficient U-Net in~\cref{subsec:kd}.
% Lastly, \revise{we introduce a method boosting generated visual quality by further fine-tuning based on FreeU~\cite{si2023freeu} in~\cref{subsec:freeu}} 


\input{tables/arch}

% \input{tables/ab_kd_short}
% \input{tables/ab_kd}
\input{tables/ab_neurips}


\subsection{Efficient U-Net architecture}\label{subsec:arch}
% Based on the investigation of the U-Net model budget of SDXL~\cite{podell2023sdxl} in~\cref{sec:sdxl}, we propose a simple yet efficient U-Net architecture.
% BK-SDM~\cite{kim2023bksdm} also compresses the U-Net of SDM-v1.4~\cite{sdm-v1.4} by removing a pair of a residual block and a transformer block at each stage.
% % However, the BK-SDM approach has a limitation in that simply block-level removal~(one block pair) can only reduce SDXL's U-Net by up to 1.3B.
% However, the BK-SDM's approach is only suitable for SDM-v1.4, which has only one transformer block~(\ie, depth=1) at each stage.
% As SDXL's U-Net has a varying number of transformer blocks at each stage, as shown in~\cref{tab:arch}, simple block-level removal~(one block pair) alone can only reduce SDXL's U-Net to at most 1.7B parameters.


We devise a compressed U-Net that is more \textit{suitable} for SDXL by introducing \textit{layer-level pruning} compared to that of BK-SDM~\cite{kim2023bksdm} which uses only block-level pruning.
Similar to BK-SDM, we first remove the residual-transformer blocks pair at each stage.
Specifically, in the encoder part~(\texttt{DW-i}), each stage has two alternating pairs of a residual block and transformer blocks.
We remove the last pair of residual-transformer blocks at each stage.
In the decoder part~(\texttt{UP-i}), we remove the intermediate pair of residual-transformer blocks.
Furthermore, focusing on the fact that the majority of the parameters are concentrated on the transformer blocks at the lowest features, as shown in~\cref{fig:arch}, we reduce the number of layers (\ie, depth) in the transformer blocks from 10 to 5 or 6 at the lowest features (\ie, \texttt{DW-3}, \texttt{Mid} and \texttt{UP-1} in~\cref{fig:arch}).
As a result, we design two types of compressed U-Net, KOALA-1B and KOALA-700M.
More details of the proposed U-Nets are demonstrated in~\cref{tab:arch} and~\cref{fig:arch}.
Note that we remove  \texttt{Mid} block in KOALA-700M for additional model compression.
Our KOALA-1B model has 1.16B parameters, making it twice as compact as SDXL~(2.56B). 
Meanwhile, KOALA-700M, with its 782M parameters, is comparable in size to SDM-v2.0~(865M). 
% It's worth noting that the inference speed of KOALA-700M is two times faster than that of SDXL but is also comparable to SDM-v2.0, which generates lower-resolution images. 






\subsection{Exploring Knowledge distillation for SDXL}\label{subsec:kd}
Now we explore how to effectively distill the knowledge of U-Net in SDXL~\cite{podell2023sdxl} into the proposed compact U-Net described in~\cref{subsec:arch}.
% As a latent diffusion model~\cite{rombach2022ldm}, SDXL encodes input $x \in \real^{3\times1024\times1024}$ to latent representation $z\in \real^{4\times128\times128}$ via VAE~\cite{kingma2013vae1,rezende2014vae2} to reduce computation cost for high-resolution generation.
% The latent representation $z$ is then fed into the U-Net~\cite{ronneberger2015uent} to predict the noise~($\epsilon$), which is the most essential part of generating the image and also the most computationally intensive. We replace this U-Net in SDXL with the proposed efficient U-Net and then train the replaced U-Net through knowledge-distillation-based learning.
Prior work~\cite{kim2023bksdm} that attempts to distill an early series of stable diffusion (\ie, SDM-v1.4~\cite{sdm-v1.4}) directly follows traditional knowledge distillation literature~\cite{romero2014featkd1,heo2019featkd2}.
The compressed student U-Net model $S_\theta$ is jointly trained to learn the target task and mimic the pre-trained U-Net of SDM-v1.4 as a teacher network.
Here, the target task is the reverse denoising process~\cite{ho2020ddpm}, and we denote the corresponding learning signal as $\loss{task}$.
% and corresponding learning signals are summarized as:
% \begin{equation}
%     \loss{task} = \min_{S_\theta} \expect_{z_t, \epsilon, t, c}||\epsilon_t - \epsilon_{S_\theta}(z_t, t, c)||^2_2,
% \end{equation}\label{eq:task_loss}
% where $\epsilon_t$ is the ground-truth sampled Gaussian noise at timestep $t$, $c$ is text embedding as a condition, $\epsilon_{S_\theta}(\cdot)$ denote the predicted noise from student U-Net model, respectively.
Besides the task loss, the compressed student model is trained to match the output of the pre-trained U-Net at both output and feature levels.
$\loss{out}$ and $\loss{feat}$ represent the knowledge distillation (KD) loss at the output- and feature-level, respectively.
% The knowledge distillation (KD) loss at output- and feature-level, $\loss{out}$ and $\loss{feat}$, are formulated as:
% \begin{equation}
%     \loss{outKD} = \min_{S_\theta} \expect_{z, \epsilon, t, c}||\epsilon_{T_\theta}(z, t, c) - \epsilon_{S_\theta}(z, t, c)||^2_2,
% \end{equation}\label{eq:out_loss}
% \begin{equation}
%     \loss{featKD} = \min_{S_\theta} \expect_{z, \epsilon, c, t}||\sum_i{f_T^i(z_t, t, c)-f_S^i(z_t, t, c)}||^2_2,
% \end{equation}\label{eq:feat_loss}
% where $\epsilon_{T_\theta}(\cdot)$ denotes the predicted noise from each U-Net in the teacher model.
For designing the feature-level KD-loss, BK-SDM~\cite{kim2023bksdm} simply considers only the last feature map of the teacher $f_T^i(\cdot)$ and student network $f_S^i(\cdot)$ at each $i$ stage as follows:
\begin{equation}
    \loss{featKD} = \min_{S_\theta} \expect_{z, \epsilon, c, t}||\sum_i{f_T^i(z_t, t, c)-f_S^i(z_t, t, c)}||^2_2,
\end{equation}\label{eq:feat_loss}
where $t$ and $c$ denote given diffusion timestep and text embeddings as conditions.
% $\epsilon_{T_\theta}(\cdot)$ denotes the predicted noise from each U-Net in the teacher model.
Thus, the feature distillation approach for text-to-image diffusion models has \textbf{\textit{not been sufficiently explored}}, leaving room for further investigation.




In this work, we extensively explore feature distillation strategies to distill the knowledge from the U-Net of SDXL effectively to our efficient U-Net, KOALA-1B.
We start from a baseline trained only by $\loss{task}$ and add $\loss{featKD}$ without $\loss{outKD}$ to validate the effect of feature distillation.
More training details are described in~\cref{subsec:ex_details} and \cref{sec:app_impl}.
From the experiments as shown in~\cref{tab:ablation}, We summarize our insights into \textit{\textbf{four important findings}} as follows.




\noindent
\textbf{F1. Which feature type is effective for distillation?}
% While BK-SDM~\cite{kim2023bksdm} uses only the last feature~(LF) for feature-based knowledge distillation~(featKD), we attempt to find which type of feature is more effective for featKD among self-attention~(SA), cross-attention~(CA), feed-forward net~(FFN) in the transformer block, residual block~(Res), and the last feature~(LF) as in BK-SDM~\cite{kim2023bksdm}.
% We use only each candidate feature type at every block in every stage.
% ~\cref{tab:distill_type} summarizes the result.
% Interestingly, we find that SA shows the best performance than others.
% Additionally, all types show improvement compared to the baseline~(SD-loss) without featKD.
BK-SDM~\cite{kim2023bksdm} demonstrated that distilling the last features (\texttt{LF}) at U-Net stages benefits overall performance when applied to shallow U-Net of early SDM-v1.4~\cite{sdm-v1.4}.
However, with the increasing complexity of U-Net and its stage, relying solely on \texttt{LF} may not be sufficient to mimic the intricate behavior of the teacher U-Net.
Thus, we revisit which features provide the richest guidance for effective knowledge distillation.
We focus on key intermediate features from each stage: outputs from the
self-attention~(\texttt{SA}), cross-attention~(\texttt{CA}), and feedforward net~(\texttt{FFN}) in the transformer block, as well as outputs from convolutional residual block~(\texttt{Res}) and \texttt{LF}.
~\cref{tab:distill_type} summarizes the experimental results.
While all types of features help obtain higher performance over the naïve baseline with only the task loss, distilling \textbf{\textit{self-attention features}} achieves the most performance gain.
Considering the prior studies~\cite{kolkin2019style,shechtman2007matching,tumanyan2022splicing} which suggest that \texttt{SA} plays a vital role in capturing semantic affinities and the overall structure of images, the results emphasize that such information is crucial for the distillation process. \\
% \indent To understand the effects more clearly, we illustrate a representative example in the~\cref{fig:attention_analysis}.
% To reason about how the distilled student U-Net captures self-similarity, we perform a PCA analysis~\cite{jolliffe2016principal,tumanyan2023plug} on self-attention maps.
% Specifically, we apply PCA on self-attention maps from \texttt{SA}- and \texttt{LF}-based models and show the top three principal components in~\cref{fig:attention_analysis}-(b).
% Interestingly, in the \texttt{SA}-based model, each principal component distinctly represents individual objects (\ie, unique color assignments to each object).
% This indicates that the \texttt{SA}-based model effectively distinguishes different objects in modeling self-similarity, which plays a crucial role in accurately rendering the distinct appearance of each object.
% In contrast, the \texttt{LF}-based model exhibits less distinction between objects, resulting in \textit{appearance leakage} between them~(\eg, a small hippo with rabbit ears).
\noindent
\textbf{F2. Which stage is most effective for distillation?}
% Considering DW1 through DW3 as the encoder part and UP1 through UP3 as the decoder part, We investigate which stage is more effective.
% We distill the SA feature only at each stage~(\eg, DW-2), ablating the other location.
% \cref{tab:distill_loc} shows that distilling knowledge at the UP1~($32\times32$) is the best.
% Furthermore, we find that the decoder part~(UP1-3) performs better than the encoder~(DW1-3), demonstrating that the decoder part plays a more essential role in the generation task. 
% Therefore, we select more SA blocks in the decoder than in the encoder for distillation as shown in~\cref{fig:arch}.
% \TODO{Add more explanation, analysis, and speculation}
% Based on the findings that self-attention features are crucial for distillation, we further explore the role and significance of each self-attention stage. 
% Intuitively, to denoise the input, the encoder of U-Net is responsible to understand semantics from noised input, while the decoder focuses on image generation by predicting noises.
% The visualization of the self-attention map, shown in ~\cref{fig:attention_analysis}-(c), back up and align with this intuition.
% Based on the first finding~(F1), we further explore the role and significance of each self-attention stage. 
% To this end, we first visualize the self-attention map in ~\cref{fig:attention_analysis}-(c).
% The self-attention maps initially capture general contextual information (\eg, \texttt{DW-2\&DW-3}) and gradually focus on localized semantics (\eg, \texttt{MID}). 
% In the decoder, self-attentions increasingly correlate with higher-level semantics (\eg, object) to accurately model appearances and structures.
% Notably, in this stage, the \texttt{SA-}based model attends corresponding object regions~(given the query patch, red box) more \textit{discriminatively} than the \texttt{LF-}based model, which results in improved compositional image generation performance.
% Building on this insight, 
In addition, we ablate the significance of each self-attention stage in the distillation process.
Specifically, we adopt an \texttt{SA-}based loss at a single stage alongside the task loss.
As shown in \cref{tab:distill_loc}, the results align with the above understanding: distilling self-attention knowledge within the \textbf{\textit{decoder}} stages significantly enhances generation quality. 
In comparison, the impact of self-attention solely within the encoder stages is less pronounced. 
Consequently, we opt to retain more \texttt{SA} layers within the decoder (see \cref{fig:arch}).
% (i.e., transformer blocks)



\noindent
\textbf{F3. Which SA's location is effective in the transformer blocks?}
At the lowest feature level, the depth of the transformer blocks is 6 for KOALA-1B, so we need to decide which locations to distill from the 10 transformer blocks of teacher U-Net.
% in SDXL with 10 transformer blocks.
% We assume three cases; case.1 \texttt{SA-bottom}: $\sum_{i=1}^Nf^i(\cdot)$, case.2 \texttt{SA-interleave}: $\sum_{i=2n+1}^{2N}f^i(\cdot)$, and case.3 \texttt{SA-up}: $\sum_{i=10-N}^{10}f^i(\cdot)$
We assume three cases for each series of transformer blocks; (1) \texttt{SA-bottom}: $ \{ f_T^l \mid l\in\{1,2,3,4,5\}\}$, (2) \texttt{SA-interleave}: $ \{ f_T^{l} \mid l \in \{1,3,5,7,9,10\} \}$, and (3) \texttt{SA-up}: $ \{ f_T^l \mid l \in \{6,7,8,9,10\} \}$ where $l$ is the number of block.
% Please refer to the illustration in the Appendix for more details.
\cref{tab:sa_loc} shows that \texttt{SA-bottom} performs the best while \texttt{SA-up} performs the worst.
This result suggests that the features of the early blocks are more significant for distillation.
% A more empirical analysis is described in~\cref{sec:app_cos}. 
% This result suggests that when the representation changes between blocks, the early transformers are less disparate.
Therefore, we adopt the \texttt{SA-bottom} strategy in all experiments.




\noindent
\textbf{F4. Which combination is the best?}
In SDXL's U-Net, as shown in~\cref{fig:arch}, there are no transformer blocks at the highest feature levels (\eg, \texttt{DW-1\&UP-3}); consequently, self-attention features cannot be distilled at this stage.
Thus, we try two options: the residual block~(\texttt{Res at DW-1\&UP-3}) and the last feature~(\texttt{LF at DW-1\&UP-3}) as BK-SDM~\cite{kim2023bksdm}.
To this end, we perform SA-based feature distillation at every stage except for \texttt{DW-1} and \texttt{UP-3}, where we use the above two options, respectively.
In addition, we try additional combinations: \texttt{SA+LF all}, \texttt{SA+Res all}, and \texttt{SA+CA+Res+FFN+LF all} where \texttt{all} means all stages.
% \cref{tab:combination} demonstrates that adding more feature distillations to SA-baed distillation consistently boots performance, and especially \texttt{LF at DW1\&UP3} shows the best.
\cref{tab:combination} demonstrates that adding more feature distillations to the SA-absent stage~(\eg, \texttt{DW-1\&UP-3}) consistently boots performance, and especially \texttt{LF at DW1\&UP3} shows the best.
Interestingly, both \texttt{+LF all} and \texttt{+Res all} are worse than the ones at only \texttt{DW-1}\&\texttt{UP-3} and \texttt{SA+CA+Res+FFN+LF all} is also not better, demonstrating that the SA features are not complementary to the other features.

With these findings, we build a \textbf{K}n\textbf{O}wledge-distill\textbf{A}tion-based \textbf{LA}tent diffusion model with our efficient U-Nets, called KOALA.
We train our KOALA models with the following objectives: $\loss{task} + \loss{outKD} + \loss{featKD}$ where we apply our findings to $\loss{featKD}$. 
% As shown in~\cref{tab:arch}, we design two models, KOALA-1B and KOALA-700M, based on SDXL~\cite{podell2023sdxl}, with U-Net model sizes of 1.16B and 782M, respectively.














% \subsection{FreeU-based fine-tuning}\label{subsec:freeu}


==> template/cvpr23/sec_short/4_experiments.tex <==


\section{Experimental results}
\vspace{-0.2cm}

\input{tables/main_table_short}

\textbf{Implementation details.} \label{subsec:ex_details}
We train the proposed efficient U-Net in SDXL~\cite{podell2023sdxl} for 200K iterations with a batch size of 128 on publicly available LAION-Aesthetics V2 6+~\cite{schuhmann2022laion-5b,laion-aesthetics,laion-aesthetics-6plus} for reproducibility.
For a fair comparison to our counterpart BK-SDM~\cite{kim2023bksdm}, we train our efficient U-Nets with their distillation method under the same data setup~(\eg, BK-SDXL-1B and -700M in~\cref{tab:main_result_short}).
% Furthermore, we also train BK-Base and BK-Small backbones in BK-SDM~\cite{kim2023bksdm} with our approach~(Ours-SDM-Base \& Ours-SDM-Small in~\cref{tab:hps_compbench}), following the BK-SDM training recipe.
More training details are described in~\cref{sec:app_impl}.


\noindent
\textbf{Evaluation metric.}
Recently, several works~\cite{betzalel2022fid_not_good,wu2023hpsv2,podell2023sdxl} have claimed that FID~\cite{heusel2017fid} is not closely correlated with visual fidelity.
Therefore, instead of FID, we use Human Preference Score~(HPSv2)~\cite{wu2023hpsv2} as a visual aesthetics metric.
For image-text alignment, we use the T2I-compbench~\cite{huang2023compbench}, which is a more comprehensive benchmark than CLIP score~\cite{hessel2021clipscore}.



% \input{tables/bk_comparison}

\input{figures/latency_gpu_11g}

\subsection{Main results}
\vspace{-0.2cm}

% \noindent 
% \textbf{Visual aesthetics.}
% Comparison to BK-SDXL & BK-SDM
We compare our KOALA-700M/1B models with popular open-sourced Stable diffusion models series~\cite{sdm-v1.4,sdm-v2.0,podell2023sdxl} and DALLE-2~\cite{ramesh2022dalle2} in~\cref{tab:main_result_short}.
Our KOALA-700M \& KOALA-1B models based on SDXL~\cite{podell2023sdxl} consistently achieve both higher HPS and CompBench average scores than the BK~\cite{kim2023bksdm} models (BK-SDXL-700M \& 1B) equipped with our efficient U-Net.
% These results demonstrate that our knowledge distillation is more general and effective than BK~\cite{kim2023bksdm}.
% These results demonstrate that the proposed distillation of the self-attention layer is more helpful for visual aesthetics than the last layer feature distillation by BK~\cite{kim2023bksdm}.
Furthermore, our KOALA-700M surpasses SDM-v2.0~\cite{sdm-v2.0} with a comparable U-Net size, which is widely used in the community.
In addition, our KOALA models show higher HPS but lower Compbench than DALLE-2~\cite{ramesh2022dalle2}, which has a much larger model size~(6.5B).
We speculate that the different tendency between DALLE-2 and our model may stem from data used for training.
Because the LAION-Aesthetics data we used focuses on higher aesthetic images than multiple objects with various attributes, our model is vulnerable to texts with different attribute properties.
% We provide more qualitative comparisons to other models, supporting the quantitative results, in~\cref{sec:app_samples}.
Lastly, when measuring latency and memory usage on a consumer-grade GPU~(\eg,11GB of VRAM), as shown in~\cref{fig:latency_gpu_11g}, SDXL cannot run with FP32 precision, whereas our KOALA-700M operates twice as fast using both FP16 and FP32 precision, showing speeds comparable to SDM-v2.0. 
% More comparisons of budgets on various GPUs are presented in~\cref{sec:app_gpus}.


==> template/cvpr23/sec_short/6_conclusion.tex <==
\vspace{-0.2cm}
\section{Conclusion and Future works}

In this work, we propose KOALA, an efficient text-to-image synthesis model, offering a compelling alternative between SDM-v2.0 and SDXL in resource-limited environments.
To achieve this, we devise more compact U-Nets and explore effective knowledge distillation strategies.
With these contributions, our KOALA-700M model substantially reduces the model size (69\%$\downarrow$) and the latency (60\%$\downarrow$) of SDXL while exhibiting decent aesthetic generation quality.

For future works, as the recent step-distillation methods~(\eg, SDXL-Turbo~\cite{sauer2023sdxl-turbo} and LCM~\cite{luo2023lcm}) are \textbf{\textit{orthogonal}} to our approach, it is expected that integrating our efficient KOALA U-Net as a substitute for the SDXL backbone can create synergistic effects, which leads to further speed-up.

% We can also expect that using a dataset with higher resolution and superior quality images will improve its generation quality because our training dataset has rather lower resolution images~(\eg, average resolution of $580\times676$).


% For future work, we will explore more diverse datasets which have high-quality prompts.
% The LAION-aesthetics-V2 6+~\cite{laion-aesthetics-6plus} we used has some low-quality and messy captions.
% Some works~\cite{yu2022parti,dalle-3} show that making caption data richer in information improves its generation quality, so refining~(cleaning) the training caption data and synthesizing more detailed captions corresponding to each paired image by a large multimodal model~\cite{liu2023llava,liu2023improvedllava} would improve the image-text alignment capability.




% data
% high-quality image (highly aesthetic image) in Emu
% \noindent
% \textbf{Data: high-resolution and highly aesthetic image.}

% For training, we use publicly available LAION-aesthetics-V2 6+~\cite{laion-aesthetics-6plus} dataset due to its easy access and reproducibility; however, the data have two limitations: 1) low resolution and 2) low-quality caption.
% Our model needs to be trained with a resolution of $1024\times1024$, but the data used for training have many images with a resolution smaller than 1024~(\eg, average solution of $580\times676$).
% Thus, as ~\cite{dai2023emu} emphasized, it will be improved by collecting higher resolution and highly aesthetic images.
% Also, the text prompts in the LAION data we used have relatively shorter and some messy texts~(\eg, HTML).
% As some works~\cite{yu2022parti,dalle-3} show that making caption data richer in information improves its generation quality, refining~(cleaning) the training caption data and synthesizing more detailed captions corresponding to each paired image by a large multimodal model~\cite{liu2023llava,liu2023improvedllava} would improve the image-text alignment capability.



% high-quality caption in Parti and DALLE-3


